Learning to Segment Medical Images from Few-Shot Sparse Labels

In this paper, we propose a novel approach for few-shot semantic segmentation with sparse labeled images. We investigate the effectiveness of our method, which is based on the Model-Agnostic Meta-Learning (MAML) algorithm, in the medical scenario, where the use of sparse labeling and few-shot can alleviate the cost of producing new annotated datasets. Our method uses sparse labels in the meta-training and dense labels in the meta-test, thus making the model learn to predict dense labels from sparse ones. We conducted experiments with four Chest X-Ray datasets to evaluate two types of annotations (grid and points). The results show that our method is the most suitable when the target domain highly differs from source domains, achieving Jaccard scores comparable to dense labels, using less than 2% of the pixels of an image with labels in few-shot scenarios.

==> SIBGRAPI - MetaLearning Medical/sec1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% Medical images are useful tools to assist doctors in multiple scenarios. Magnetic resonance imaging (MRI), computed tomography (CT), and other imaging are less invasive methods that allow doctors to analyze the anatomy of an object of interest, for example an organ, a tissue, or a tumor.
% Semantic segmentation delimit objects in the images, and such delimitation of structures in medical images can help in diagnosis, pathology localization, anatomical studies, and other tasks~\cite{sharma2010automated}.

Medical images are useful tools to assist doctors in multiple clinical scenarios and to plan for surgery. X-Ray, Magnetic Resonance Imaging (MRI), Computed Tomography (CT) and other imaging modalities are non-invasive methods that %combined with semantic segmentation delimiting objects in the images,
can help in diagnosis, pathology localization, anatomical studies, and other tasks~\cite{sharma2010automated}.

Convolutional Neural Networks (CNNs) and their variants are the state of the art for object classification, detection, semantic segmentation and other Computer Vision problems. Classical convolutional networks are known for their large data requirements, often hindering their usage in scenarios were data availability is limited, as in medical imaging. Relatively few medical datasets are publicly available due to privacy and ethical concerns \cite{shiraishi2000development,jaeger2014two,NIHwang2017chestx,MIASsuckling1994mammographic,IVISIONsilva2018automatic,PANORAMICabdi2015automatic,moreira2012inbreast}.

Even among the public datasets, properly curated labeled data is limited due to the need for specialized annotators (i.e. radiologists), severely hampering the creation of general models for medical image understanding. While many datasets contain image-level annotations indicating the presence or absence of a set of medical conditions, the creation of pixel-level labels that allow for the training of semantic segmentation models is much more laborious. Volumetric image modalities as MRIs or CT scans further compound these difficulties by requiring per-slice annotations, often followed by cross-axes analysis to detect inconsistencies, which can take hours for one single exam. Hence, there is a need for automatic and semi-automatic segmentation methods to assist physicians in the annotation of these images. One way to alleviate the burden of medical professionals in labeling the exams is to improve the generalization capabilities of existing pretrained models. For instance, domain adaptation can be used to transfer knowledge from related medical imaging datasets to improve segmentation performance in unseen target tasks. % One must provide a label for every pixel in the image, which is laborious, and in the medical case, most likely, a specialist is required to annotate the data.
% \todo{(PESSIMA FRASE) As Deep Neural Networks (DNNs), in specific the convolutional models (CNNs), becoming state-of-the-art for segmentation, their larger requirement of data appears as a problem in the development of solutions using these methods in areas were data is scarce, for example, in medical scenarios. 
% (INSERIR ALGO SOBRE CUSTO DE CONSTRUIR DATASETS: ACHAR IMG, ESPECIALISTA, ETC)
% The few publicly available medical datasets, such as JSRT~\cite{shiraishi2000development} and Montgomery/Shenzhen dataset~\cite{jaeger2014two} have a small amount of data, and this can difficult the creation of more general models.}
% FIRST VERSION 
% To further improve the usefulness of such images, different process are applied to these data. One of these process is the segmentation, that perform a delineation  of objects in images. The delimitation of the structures can help in diagnosis, pathology localization, anatomical studies, and other tasks.\todo{add refs}

% Different process can be applied to the raw data that can improve their use to medical professionals. One of such process is segmentation, that is to divide an image in different semantic objects. The delimitation of the structures can help in diagnosis, pathology localization, anatomical studies, and other tasks~\cite{sharma2010automated}.

% The semantic segmentation task is a classical problem in the computer vision area, that nowadays is mostly tackled by methods using Convolutional Neural Networks (CNNs). These models have been proven efficient in tasks, such as classification, with common photographs . As expected, different works applied CNN methods to medical images~\cite{nie2016fully, gibson2018automatic, gordienko2017,  skourt2018lung}.

% The task of semantic segmentation is a classical problem in computer vision. In recent years, methods using Convolution Neural Networks (CNNs \cite{lecun1990handwritten}) became the state-of-the-art to this problem in many cases, as seen in different benchmarks\footnotemark\footnotetext{\url{https://www.cityscapes-dataset.com/benchmarks/}} or competitions\footnotemark\footnotetext{\url{http://cocodataset.org/\#panoptic-leaderboard}}. As expected, in recent years different works applied CNN methods to medical imaging producing relevant results~\cite{nie2016fully,gibson2018automatic,gordienko2017,skourt2018lung}.

% Convolution Neural Networks (CNNs \cite{lecun1990handwritten}) are the state-of-the-art in semantic segmentation.  %In recent years different works applied CNN methods to medical imaging producing relevant results~\cite{nie2016fully,gibson2018automatic,gordienko2017,skourt2018lung}.
% One common problem with CNNs, and deep learning methods, in general is their requirement of large volumes of data. The labeling process necessary to produce semantic segmentation data is laborious and, in medical image, usually, requires a specialist. Thus, these dataset are usually expensive to produce. Publicly available medical datasets, such as JSRT~\cite{shiraishi2000development} and Montgomery/Shenzhen dataset~\cite{jaeger2014two} have a small amount of data, and this can hinder the creation of more general models.

% One problem with the usual CNN methods is the necessity of large amounts of data, and more specifically annotated data. As the labeling of images normally require a specialists, such data is expensive to produce, and the publicly available options, such as \todo{refs}, do not cover a large array of tasks.

% Overall, usual CNN methods - deep learning methods, in general - perform poorly with small amount of data, specifically annotated data. The labeling process necessary to produce semantic segmentation data is laborious and, in most cases, requires a specialist. Thus, these dataset are usually expensive to produce. Publicly available medical datasets, such as JSRT~\cite{shiraishi2000development} and Montgomery/Shenzhen dataset~\cite{jaeger2014two} have a small amount of data that can hinder the creation of more general models.

% To circumvent these problem, we will approach the task of image segmentation with the Few-shot paradigm. This paradigm is useful when only a small(e.g., less than 50 images) amount of data is available. The works \todo{refs} explore methods in these scenarios, for classification. Furthermore, this work will utilize sparse labels. This labeling approach differs from the usual in the way that the later requires all pixels in an image to have an associated class label, as opposed to our scenario where only a few pixels have such labels.

% As a problem that affects deep learning methods in general, these cases where small data are available has recently gained interest in the scientific community. Also called Few-Shot scenarios, these cases have been studied for different tasks, for example, the works \cite{vinyals2016matching, snell2017prototypical, finn2017model} proposes methods to Few-Shot classification problems. 

% Few-shot scenarios, where low amounts of data are available, have been studied for different tasks, such as classification~\cite{snell2017prototypical,finn2017model}, in recent years.
% Annotating an entire image for semantic segmentation labeling is time-consuming.
% An efficient option is \textit{sparse labeling}, that is, specifying the labels of a small number of pixels. Such annotations can be challenging to work, but can produce results comparable to full labeling. The joined use of few-shot and sparse labeling can reduce the cost of producing semantic segmentation medical datasets.
Scenarios with low amounts of data available, often called Few-shot, have been studied in recent years. Tasks such as few-shot classification~\cite{snell2017prototypical,finn2017model} are the most explored in the literature with substantial results for datasets such as MNIST \cite{lecun1998gradient} or Omniglot \cite{lake2015human}. As for the problem of pixel-level annotations, one efficient option is \textit{sparse labeling}, that is, specifying the labels of a small number of pixels. Methods that can make efficient use of few-shot and sparse labels can solve semantic segmentation medical problems on datasets created in a labor-efficient manner.
Thus, \textbf{our main contribution} is the proposal of a novel approach to few-shot semantic segmentation in medical images from sparse labels. For that, we introduce the \textbf{Wea}kly-supervised \textbf{Se}gmentation \textbf{L}earning (WeaSeL), which extends the MAML~\cite{finn2017model} algorithm by introducing annotation sparsity directly to its meta-training stage.
% Secondary contributions include: 1) a thorough evaluation of Meta-Learning for few-shot sparse segmentation on several distinct scenarios; and 2) an assessment of label efficiency in point and grid labeling configurations. %; 3) a standardized meta-dataset for radiogram segmentation from sparse labels.
% \begin{itemize}
%     % \item A thorough evaluation of sparse labeling configurations using Guided Networks \cite{rakelly2018conditional};
%     \item A standardized Meta-Dataset composed of several organ segmentation tasks in radiological images;
%     \item 
% \end{itemize}
% Moreover, we perform an extensive evaluation of this method in different datasets ands tasks.

% \todo{Introduce the commonly used sparse labeling styles.}

==> SIBGRAPI - MetaLearning Medical/sec2_related.tex <==
\section{Related Work}
\label{sec:related}

% FIRST VERSION
% Automatic segmentation of medical images has been studied for many years. Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. \citet{nie2016fully} uses a Fully Convolutional Neural Network (FCN)~\cite{long2015fully} to segment brain tissue in infants. The authors propose an architecture to segment Magnetic Resonance imaging (MRI) of brains in in 4 categories: white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF) and background. \citet{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net. They use this network to perform multiple organs segmentation in 3d abdominal Computed tomography (CT) imaging. In~\cite{gordienko2017} the authors studies lungs segmentation. They use an U-Net \cite{ronneberger2015u} architecture to segment lungs from the background in XRay images from the JSRT dataset~\cite{shiraishi2000development}. In a similar procedure,~\cite{skourt2018lung} also performs lung segmentation. In this work, they train an U-Net in the Lung Image Database Consortium image collection (LIDC-IDRI)~\cite{lidc-idri}.

\noindent\textbf{Biomedical Image Segmentation:} Automatic and semi-automatic segmentation of medical images has been studied for decades, as such methods can considerably alleviate the burden of physicians in labeling these data \cite{ronneberger2015u}. Medical image segmentation from sparse labels can be especially useful, since these images often have a small number of labeled samples due to data privacy restrictions and the lack of specialists for annotating the samples. The survey of Tajbakhsh \textit{et. al} \cite{tajbakhsh2020embracing} reviews a collection of Deep Learning (DL) solutions on medical image segmentation, which includes a section for segmentation with noisy/sparse labels. The methods reviewed can be summarized in a selective loss with or without mask completion. Sparse segmentation methods either use a loss function able to ignore unlabeled pixels/voxels or employ some technique to augment the sparse annotations to resemble dense masks.

% Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. 
% The works \cite{nie2016fully,gibson2018automatic,gordienko2017,skourt2018lung} use a variation of a CNN to segment various type of medical images. In \cite{gordienko2017,skourt2018lung} they use an U-Net~\cite{ronneberger2015u} architecture, while \cite{nie2016fully} uses an Fully Convolutional Network(FCN)~\cite{long2015fully}, and \cite{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net, similar to an U-Net. 
% Both \cite{gordienko2017,skourt2018lung} perform lung segmentation in different types of images. \cite{gordienko2017} work with XRay images from JSRT dataset~\cite{shiraishi2000development} and \cite{skourt2018lung} Computed Tomography(CT) images from LIDC-IDRI~\cite{lidc-idri}.~\cite{gibson2018automatic} also use CT images, but from abdominal region, while \cite{nie2016fully} focus on Magnetic Resonance Imaging(MRI) of infant brains. 

% \todo{Mention the survey on medical image segmentation with noisy/sparse labels by \cite{tajbakhsh2020embracing}. Use taxonomy to define our methodology. Provide a table in the related work organizing the referenced papers using the taxonomy.}

% The survey of Tajbakhsh et. al~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation. This survey includes a section for segmentation with noisy/sparse labels. The methods for sparse label can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse, bai2018recurrent, cai2018accurate, can2018learning, matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, e.g.~\cite{cciccek20163d, silvestri2018stereology, bokhorst2018learning, zhu2019pick} -- \cite{cciccek20163d, bokhorst2018learning} using a weighted loss, \cite{silvestri2018stereology} implies the use of padding in the sparse labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based of the sparse annotation.

% The innate nature of semantic segmentation makes sparse labeling a challenging scenario.~\cite{vernaza2017learning} approach this case with a label propagation scheme. The authors propose an two branch pipeline, one of an ordinary segmentation network and the other a label propagation using random-walk. During training the two branches are expected to agree on the pixel classification.~\cite{cciccek20163d} proposes a much simpler method to sparse label scenarios. Working with 3D images of \textit{Xenopus} embryos with only a few annotated voxels, the authors reweight the importance of diferent classes in the objective function. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are ignored when computing the training loss.

% \subsection{Meta-Learning for Few-Shot Scenarios}
% \label{sec:meta_learning}

% In recent years, many works had focused on Few-Shot scenarios, specifically for the classification task. The works \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} can be seen as a form of Metric Learning approach, were the models learn embedding functions to a space different of the input (REVISION NEEDED). \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses the support set - the set of few labeled images - to guide its transformation, than the model uses a weighted average to predict the class probability of the query image (e.g. the image of interest, in this task, an image to be classified). \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets). This model tries to learn em embedding function that computes \textit{prototypes} to a class (e.g. a $d$-dimensional vector that represents a class). When predicting a query image class, the model computes its prototype and compares with the class prototypes produced by the support set, being the closest one assigned as the predicted label. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs). Their model, learns to create an $d$-dimensional subspace from the support set, for each class. A query image is than embedded to this space and the distance of their projection to each subspace is computed. The subspace with the smaller projection distance is chosen as the class of the query.

% There have been an increasingly use of meta-learning to Few-Shot scenarios, primarily classification. Generally, these methods can be divided in metric learning and optimization approaches. The former focusing on models learning embedding functions, and computing distances in the embedding spaces. The later focusing in new methods to direct optimize models in this data regime.

% \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} are examples of Metric Learning approaches. \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses a small set of images to guide its transformation. \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets), a model that tries to learn em embedding function that computes \textit{prototypes} to a class (e.g. a $d$-dimensional vector that represents a class) and uses these distance to these prototypes for inference. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs), a model that learns to create an $d$-dimensional subspace from the support set, for each class, and the projection distance to these subspaces are used for class prediction. 

% A different strategy can be seen in the works \cite{finn2017model, raghu2019rapid, yoon2018bayesian, finn2018probabilistic}, that can be described as Gradient-Based, that is algorithms that proposes novel gradient optimizations to train models in this data regime (REVISION NEEDED). In \cite{finn2017model} the authors proposed the MAML framework. In this framework they use multiple tasks (an small data sample for train/test with an loss function). They train the model to generalize well to these tasks. 
% There is an \textit{outer} an \textit{inner} loop in the training process. The outer loop, an global parameter $\Theta$ is optimized to provide good initialization parameters for specific tasks. In the inner loop, the model takes the global $\Theta$ and create a $\Theta_i$ specific to each task sampled in that outer loop iteration, producing a task specific loss based of them. The summation of these losses is than used to compute the gradients to the global $\Theta$.
% % There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
% The work~\cite{raghu2019rapid} is an modification of the MAML~\cite{finn2017model} model. The novel proposed by \cite{raghu2019rapid} is that in the \textit{inner} loop of MAML, instead of updating all the $\Theta$ parameters, they only update the parameters related to the network head (the components of the network that are correspondent to an classifier, in this case). With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) \cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop. \cite{finn2018probabilistic} presents an probabilistic version of MAML. The $\Theta$ parameters are not the weights of an network, but instead they define a distribution over such weights. During training, in the inner loop, they use information over the test set of a task to sample the weights that will be updated for a task. The outer loop loss also include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

\noindent\textbf{Meta-Learning:} Few-shot learning has attracted considerable attention over the last years, mainly due to recent advances in Deep Learning for Self-Supervised learning \cite{goyal2019scaling} and Meta-Learning \cite{snell2017prototypical,finn2017model}. Meta-Learning has become a proliferous research topic in Deep Learning, as the literature aims to improve on the generalization capabilities of Deep Neural Networks (DNNs). Within Meta-Learning, two prominent and distinct methodologies gained attention: Gradient-based and Metric learning. Finn \textit{et al.} \cite{finn2017model} proposed the MAML framework, based on the trend of Gradient-based approaches. MAML uses multiple tasks -- that is, multiple data/sample pairs and a loss function -- during its meta-training to create a generalizable model able to perform quick adaptation and feature reuse to infer over unseen related tasks. 
% More details on MAML can be seen in Section~\ref{sec:methodology}. 
Meta-Learning arose at first for object classification tasks, while tasks such as detection and segmentation still lacking development. Additionally, the intersection of few-shot learning and medical image segmentation from sparse labels has proven to be quite a challenging task, with very few methods being described in the literature \cite{wang2018interactive}.
%Gradient-based Meta-Learning often has two nested loops: an \textit{inner} loop that tries to minimize the loss of a specific task, and an \textit{outer} while the outer the model parameters are optimized to be generally usable for all tasks. 
% There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
% Raghu \textit{et al.} \cite{raghu2019rapid} evaluated the capabilities of MAML in order to determine if Gradient-based Meta-Learning relies more on feature reuse or quick adaptability, resulting in the Almost No Inner Loop (ANIL) methodology, wherein only the classification head of the network is optimized during the \textit{inner} loop. % is an modification of the MAML algorithm, which consists in only update the parameters related to the network head (the components of the network that are equivalent to a classifier, in this case) within the \textit{inner} loop, instead of all the model parameters.
% With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) 
% \cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop.
% \cite{finn2018probabilistic} presents an probabilistic version of MAML. The parameters of the model define a distribution over such weights of a network. In the outer loop, they include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

% \subsection{Semantic Segmentation from Sparse Labels}
% \label{sec:sparse_seg}

% \todo{Mention \cite{lin2016scribblesup} as a precursor in the area. Does not rely on meta-learning, modern DA, etc. Simply works with a standard FCN, label propagation and pre-training.}

% One of the first works to use sparse labels for semantic segmentation is \cite{lin2016scribblesup}, where they use a scheme of label propagation from the scribble annotations in conjunction with a FCN for segmentation. \cite{wang2018interactive} uses a principle similar to \cite{lin2016scribblesup}, but applied to biomedical images. The difference is that the model is trained on full annotations, and then the model iteratively refines their segmentation for an image, possibly using scribbles provided by the user interactively.  

% \todo{Mention the paper by \cite{wang2018interactive} about interactive sparse-labeled segmentation for biomedical images.}

% Moreover, the survey of Tajbakhsh et. al~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation, which includes a section for segmentation with noisy/sparse labels. The methods reviewed can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse, bai2018recurrent, cai2018accurate, can2018learning, matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, e.g.~\cite{cciccek20163d, silvestri2018stereology, bokhorst2018learning, zhu2019pick} -- \cite{cciccek20163d, bokhorst2018learning} using a weighted loss, \cite{silvestri2018stereology} implies the use of padding of labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based on sparse annotations.

% \subsection{Few-Shot Semantic Segmentation}
% \label{sec:few_shot_seg}

% FIRST VERSION
% Few-shot semantic segmentation is a field that only recently started to be explored.~\citet{shaban2017one} proposes a method to few-shot segmentation. A two-branch network is used, one branch is a usual segmentation network, such as FCN, the other branch receives an support set of images and produce weights. This weights are  used in the other branch to perform the final segmentation.~\citet{dong2018few} introduces an architecture for few-shot semantic segmentation based on the prototypical networks~\cite{snell2017prototypical}, that were originally proposed for classification. Their framework is divided in two network. One is used to produce the prototypes for each class in the query image using the support set. The second produces a feature map from the query image, this map is weighted using the prototypes. The weighted feature map is than used to produce the final segmentation.~\citet{rakelly2018conditional} is similar to \cite{shaban2017one}. The difference is that in \cite{rakelly2018conditional} the authors use the same network to extract the features from the query and support images. The features of the support images are further use to "guide" the segmentation of the query image, that is, these features are aggregated to the ones of the query image, and then processed to generate the segmentation. The works~\cite{dong2018few, shaban2017one, rakelly2018conditional} were firstly proposed to usual photographs. \citet{zhao2019data} tackled one-shot segmentation in brain MRIs. The authors proposed a framework where they use CNN to learn transformations that can be used to data augment their dataset. With the trained networks and a single annotated image, they synthesize a dataset from unlabeled brain MRIs. This dataset is then used to train a network in a supervised fashion.

% Few-shot semantic segmentation became a relevant topic only recently. Works like \cite{shaban2017one, dong2018few, hu2019attention, zhang2019sgone, wang2019panet} present some approaches to use the support set to segment the query image. In \cite{shaban2017one} implements a simple network for the extraction of the weights from the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, that are than fused with the features extracted from the query, thus being an adaptation of the Prototypical Networks~\cite{snell2017prototypical}. \cite{zhang2019sgone} uses an masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets. The authors compute the prototypes using masked average pooling, but additionally an \textit{alignment} loss is used, where the query image is used to produce the prototypes and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. This model uses attention modules, that receive both query features, as well as masked support images features. At last, an recurrent network is used to access information of all sample in the support set and produce the final prediction. These works (\cite{shaban2017one, dong2018few, rakelly2018conditional, hu2019attention, zhang2019sgone, wang2019panet}) were firstly proposed to usual photographs as seen in datasets like the Pascal VOC~\cite{pascal-voc-2012}. \cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs. The authors use a single labeled example and a large set of unlabeled images to construct a synthetic dataset, using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

\noindent\textbf{Few-shot Semantic Segmentation:} Few-shot segmentation became a relevant topic only recently. Several methods \cite{shaban2017one,dong2018few,hu2019attention,zhang2019sgone,wang2019panet} were recently proposed to make use of the small subset of labeled images, often called \textit{support} set, to segment a query image. However, the vast majority of few-shot segmentation methods in the literature do not explore sparsely labeled images in the support set, only dealing with densely labeled samples. %Shaban \textit{et al.} \cite{shaban2017one} implements a simple network to produce weights based on the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, as the ProtoNets~\cite{snell2017prototypical}, that are than fused with the features extracted from the query. \cite{zhang2019sgone} uses a masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets, computing the prototypes using masked average pooling, but additionally include an \textit{alignment} loss, where the prototypes are computed from the query image and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. It uses attention modules, that receive both query features, as well as masked support images features. At last, a recurrent network is used to access information of all sample in the support set and produce the final prediction.
Rakelly \textit{et al.} \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation: Guided Networks.
Guided Nets use a pretrained CNN backbone to extract features of both the support set and the query image. The weakly labeled support samples and sparse segmentation masks are combined, pooled, and subsequently used as weights to segment the query. The vast majority of few-shot segmentation methods  \cite{shaban2017one,dong2018few,rakelly2018conditional,hu2019attention,zhang2019sgone,wang2019panet} were originally proposed to RGB images as the ones seen in datasets such as the Pascal VOC~\cite{pascal-voc-2012}, thus, most of the literature on this topic rely on pretrained CNN or even Fully Convolutional Networks (FCNs) backbones.

% \cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs, where they construct a synthetic dataset from a single labeled image and a large unlabeled dataset using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

% In this work we did not present the Guided Nets~\cite{rakelly2018conditional} as a baseline, although being a few-shot sparse segmentation method. There were two main problems with the method. The first, being that using pretrained DNNs from ImageNet datasets were not useful for the medical imaging used. The second, was that even to the best of our efforts, the model did not converge with the episodic training used a single binary dataset (most of the medical datasets used). Since, it did not seen fair to compare the Guided Nets with our approach.
% \todo{Justify the absence of Guided Nets as a baseline: inability to use pretrained DNNs from ImageNet and problems with episodic training on binary labels from the Meta-Dataset (did not converge to the best of our efforts).}

% FIRST VERSION
% Sparse labeling segmentation can be challenging scenario.~\citet{vernaza2017learning} tackle the sparse label scenario in an interesting manner. They propose a labeling propagation scheme using random-walk. Two networks are used, one is used in the labeling propagation and the other is an ordinary segmentation network. In training, in parallel the image is segmented by one of the networks and has the sparse labels propagated to all pixels. The train objective is that these two branches agree on the final prediction.~\citet{cciccek20163d} uses a simple approach to the sparse label scenario. The authors use an UNet architecture in 3d images of \textit{Xenopus} embryos. In this work, to train the network they reweight the importance of the voxels. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are unconsidered in computing the training loss.

% Our work is uses the approach of \cite{cciccek20163d}, to deal with sparse labels. Our methods are built upon MAML \cite{finn2017model} and ProtoNets \cite{snell2017prototypical}, thus is related to CITE. The frameworks of MAML and ProtoNets will be further detailed in the section CITE, since they are essential to our methods.

% \subsection{Few-Shot Segmentation from Sparse Labels}
% \label{sec:few_shot_sparse_seg}

% % "This is a natural extension of [24] to segmentation, but we find it is difficult to optimize for structured output, perhaps due to multi-modality or fine-tuning from pre-training. [...] In comparing feature fusion, parameter regression, and prototypes we find feature fusion is more accurate and simpler to tune. This is the inference strategy used for all of our results." \cite{rakelly2018conditional}.

% All methods referenced in Section~\ref{sec:few_shot_seg} address the problem of few-shot semantic segmentation regarding the number of labeled images used in the support set, while the methods presented in Section~\ref{sec:sparse_seg}. However, none of these methods address the scenario of few-shot learning from sparse annotations, relying on laborious dense labeling masks. Dense masks may be unfeasible or undesirable for applications that depend on annotations from specialists (e.g. biomedical imaging or remote sensing).

% \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation.

% The authors of \cite{rakelly2018conditional} use the same network to extract features of the support set and the query image, but the support features are used as weights.

==> SIBGRAPI - MetaLearning Medical/sec2_related_old.tex <==
\section{Related Work}
\label{sec:related}

% FIRST VERSION
% Automatic segmentation of medical images has been studied for many years. Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. \citet{nie2016fully} uses a Fully Convolutional Neural Network(FCN)~\cite{long2015fully} to segment brain tissue in infants. The authors propose an architecture to segment Magnetic Resonance imaging (MRI) of brains in in 4 categories: white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF) and background. \citet{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net. They use this network to perform multiple organs segmentation in 3d abdominal Computed tomography(CT) imaging. In~\cite{gordienko2017} the authors studies lungs segmentation. They use an U-Net \cite{ronneberger2015u} architecture to segment lungs from the background in XRay images from the JSRT dataset~\cite{shiraishi2000development}. In a similar procedure,~\cite{skourt2018lung} also performs lung segmentation. In this work, they train an U-Net in the Lung Image Database Consortium image collection (LIDC-IDRI)~\cite{lidc-idri}.

Automatic and semi-automatic segmentation of medical images has been studied for decades, as such methods can considerably alleviate the burden of physicians in labeling these data \cite{ronneberger2015u}. Medical image segmentation from sparse labels can be especially useful, as biomedical images often have a small number of labeled samples due to data privacy restrictions and the lack of specialists for annotating the samples. Additionally, Few-Shot learning has attracted considerable attention over the last years, mainly due to recent advances in Deep Learning for Self-Supervised learning \cite{goyal2019scaling} and Meta-Learning \cite{snell2017prototypical,finn2017model}. However, the intersection of Few-Shot learning and medical image segmentation from sparse labels has proven to be quite a challenging task, with very few methods being described in the literature \cite{wang2018interactive}.
% Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. 
% The works \cite{nie2016fully,gibson2018automatic,gordienko2017,skourt2018lung} use a variation of a CNN to segment various type of medical images. In \cite{gordienko2017,skourt2018lung} they use an U-Net~\cite{ronneberger2015u} architecture, while \cite{nie2016fully} uses an Fully Convolutional Network(FCN)~\cite{long2015fully}, and \cite{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net, similar to an U-Net. 
% Both \cite{gordienko2017,skourt2018lung} perform lung segmentation in different types of images. \cite{gordienko2017} work with XRay images from JSRT dataset~\cite{shiraishi2000development} and \cite{skourt2018lung} Computed Tomography(CT) images from LIDC-IDRI~\cite{lidc-idri}.~\cite{gibson2018automatic} also use CT images, but from abdominal region, while \cite{nie2016fully} focus on Magnetic Resonance Imaging(MRI) of infant brains. 

% \todo{Mention the survey on medical image segmentation with noisy/sparse labels by \cite{tajbakhsh2020embracing}. Use taxonomy to define our methodology. Provide a table in the related work organizing the referenced papers using the taxonomy.}

% The survey of Tajbakhsh et. al~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation. This survey includes a section for segmentation with noisy/sparse labels. The methods for sparse label can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse, bai2018recurrent, cai2018accurate, can2018learning, matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, i.e.~\cite{cciccek20163d, silvestri2018stereology, bokhorst2018learning, zhu2019pick} --- \cite{cciccek20163d, bokhorst2018learning} using a weighted loss, \cite{silvestri2018stereology} implies the use of padding in the sparse labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based of the sparse annotation.

% The innate nature of semantic segmentation makes sparse labeling a challenging scenario.~\cite{vernaza2017learning} approach this case with a label propagation scheme. The authors propose an two branch pipeline, one of an ordinary segmentation network and the other a label propagation using random-walk. During training the two branches are expected to agree on the pixel classification.~\cite{cciccek20163d} proposes a much simpler method to sparse label scenarios. Working with 3D images of \textit{Xenopus} embryos with only a few annotated voxels, the authors reweight the importance of diferent classes in the objective function. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are ignored when computing the training loss.

% \subsection{Meta-Learning for Few-Shot Scenarios}
% \label{sec:meta_learning}

% In recent years, many works had focused on Few-Shot scenarios, specifically for the classification task. The works \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} can be seen as a form of Metric Learning approach, were the models learn embedding functions to a space different of the input (REVISION NEEDED). \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses the support set - the set of few labeled images - to guide its transformation, than the model uses a weighted average to predict the class probability of the query image (i.e. the image of interest, in this task, an image to be classified). \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets). This model tries to learn em embedding function that computes \textit{prototypes} to a class (i.e. a $d$-dimensional vector that represents a class). When predicting a query image class, the model computes its prototype and compares with the class prototypes produced by the support set, being the closest one assigned as the predicted label. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs). Their model, learns to create an $d$-dimensional subspace from the support set, for each class. A query image is than embedded to this space and the distance of their projection to each subspace is computed. The subspace with the smaller projection distance is chosen as the class of the query.

% There have been an increasingly use of meta-learning to Few-Shot scenarios, primarily classification. Generally, these methods can be divided in metric learning and optimization approaches. The former focusing on models learning embedding functions, and computing distances in the embedding spaces. The later focusing in new methods to direct optimize models in this data regime.

% \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} are examples of Metric Learning approaches. \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses a small set of images to guide its transformation. \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets), a model that tries to learn em embedding function that computes \textit{prototypes} to a class (i.e. a $d$-dimensional vector that represents a class) and uses these distance to these prototypes for inference. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs), a model that learns to create an $d$-dimensional subspace from the support set, for each class, and the projection distance to these subspaces are used for class prediction. 

% A different strategy can be seen in the works \cite{finn2017model, raghu2019rapid, yoon2018bayesian, finn2018probabilistic}, that can be described as Gradient-Based, that is algorithms that proposes novel gradient optimizations to train models in this data regime (REVISION NEEDED). In \cite{finn2017model} the authors proposed the MAML framework. In this framework they use multiple tasks (an small data sample for train/test with an loss function). They train the model to generalize well to these tasks. 
% There is an \textit{outer} an \textit{inner} loop in the training process. The outer loop, an global parameter $\Theta$ is optimized to provide good initialization parameters for specific tasks. In the inner loop, the model takes the global $\Theta$ and create a $\Theta_i$ specific to each task sampled in that outer loop iteration, producing a task specific loss based of them. The summation of these losses is than used to compute the gradients to the global $\Theta$.
% % There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
% The work~\cite{raghu2019rapid} is an modification of the MAML~\cite{finn2017model} model. The novel proposed by \cite{raghu2019rapid} is that in the \textit{inner} loop of MAML, instead of updating all the $\Theta$ parameters, they only update the parameters related to the network head (the components of the network that are correspondent to an classifier, in this case). With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) \cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop. \cite{finn2018probabilistic} presents an probabilistic version of MAML. The $\Theta$ parameters are not the weights of an network, but instead they define a distribution over such weights. During training, in the inner loop, they use information over the test set of a task to sample the weights that will be updated for a task. The outer loop loss also include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

The works \cite{finn2017model, raghu2019rapid, yoon2018bayesian, finn2018probabilistic}, can be seen as Optimization/Gradient-Based approaches. Finn \textit{et al.} \cite{finn2017model} propose the Model-Agnostic Meta-Learning (MAML) framework, based on the trend of Optimization/Gradient-based approaches. In this framework they use multiple tasks (an small data sample for train/test with an loss function) in training to create a general model. 
There are two nested loops(\textit{outer} an \textit{inner}) in the training process. In the inner loop the model is optimized to minimize the loss of a task, while the outer the model parameters are optimized to be generally usable for all tasks. 
% There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
The work~\cite{raghu2019rapid} is an modification of the MAML algorithm, which consists in only update the parameters related to the network head (the components of the network that are equivalent to a classifier, in this case) within the \textit{inner} loop, instead of all the model parameters.
% With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) 
\cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop.
\cite{finn2018probabilistic} presents an probabilistic version of MAML. The parameters of the model define a distribution over such weights of a network. In the outer loop, they include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

% \subsection{Semantic Segmentation from Sparse Labels}
% \label{sec:sparse_seg}

% \todo{Mention \cite{lin2016scribblesup} as a precursor in the area. Does not rely on meta-learning, modern DA, etc. Simply works with a standard FCN, label propagation and pre-training.}

One of the first works to use sparse labels for semantic segmentation is \cite{lin2016scribblesup}, where they use a scheme of label propagation from the scribble annotations in conjunction with a FCN for segmentation. \cite{wang2018interactive} uses a principle similar to \cite{lin2016scribblesup}, but applied to biomedical images. The difference is that the model is trained on full annotations, and then the model iteratively refines their segmentation for an image, possibly using scribbles provided by the user interactively.  

% \todo{Mention the paper by \cite{wang2018interactive} about interactive sparse-labeled segmentation for biomedical images.}

Moreover, the survey of Tajbakhsh \textit{et. al}~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation, which includes a section for segmentation with noisy/sparse labels. The methods reviewed can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse,bai2018recurrent,cai2018accurate,can2018learning,matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, e.g.~\cite{cciccek20163d,silvestri2018stereology,bokhorst2018learning,zhu2019pick} --- \cite{cciccek20163d,bokhorst2018learning} using a weighted loss, Silvestri \textit{et al.} \cite{silvestri2018stereology} implies the use of padding of labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based on sparse annotations.

\subsection{Few-Shot Semantic Segmentation}
\label{sec:few_shot_seg}

% FIRST VERSION
% Few-shot semantic segmentation is a field that only recently started to be explored.~\citet{shaban2017one} proposes a method to few-shot segmentation. A two-branch network is used, one branch is a usual segmentation network, such as FCN, the other branch receives an support set of images and produce weights. This weights are  used in the other branch to perform the final segmentation.~\citet{dong2018few} introduces an architecture for few-shot semantic segmentation based on the prototypical networks~\cite{snell2017prototypical}, that were originally proposed for classification. Their framework is divided in two network. One is used to produce the prototypes for each class in the query image using the support set. The second produces a feature map from the query image, this map is weighted using the prototypes. The weighted feature map is than used to produce the final segmentation.~\citet{rakelly2018conditional} is similar to \cite{shaban2017one}. The difference is that in \cite{rakelly2018conditional} the authors use the same network to extract the features from the query and support images. The features of the support images are further use to "guide" the segmentation of the query image, that is, these features are aggregated to the ones of the query image, and then processed to generate the segmentation. The works~\cite{dong2018few, shaban2017one, rakelly2018conditional} were firstly proposed to usual photographs. \citet{zhao2019data} tackled one-shot segmentation in brain MRIs. The authors proposed a framework where they use CNN to learn transformations that can be used to data augment their dataset. With the trained networks and a single annotated image, they synthesize a dataset from unlabeled brain MRIs. This dataset is then used to train a network in a supervised fashion.

% Few-shot semantic segmentation became a relevant topic only recently. Works like \cite{shaban2017one, dong2018few, hu2019attention, zhang2019sgone, wang2019panet} present some approaches to use the support set to segment the query image. In \cite{shaban2017one} implements a simple network for the extraction of the weights from the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, that are than fused with the features extracted from the query, thus being an adaptation of the Prototypical Networks~\cite{snell2017prototypical}. \cite{zhang2019sgone} uses an masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets. The authors compute the prototypes using masked average pooling, but additionally an \textit{alignment} loss is used, where the query image is used to produce the prototypes and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. This model uses attention modules, that receive both query features, as well as masked support images features. At last, an recurrent network is used to access information of all sample in the support set and produce the final prediction. These works(\cite{shaban2017one, dong2018few, rakelly2018conditional, hu2019attention, zhang2019sgone, wang2019panet}) were firstly proposed to usual photographs as seen in datasets like the Pascal VOC~\cite{pascal-voc-2012}. \cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs. The authors use a single labeled example and a large set of unlabeled images to construct a synthetic dataset, using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

Few-shot semantic segmentation became a relevant topic only recently. Works like \cite{shaban2017one, dong2018few, hu2019attention, zhang2019sgone, wang2019panet} present some approaches to use the \textit{support set} --- the small set of labeled images --- to segment a query image. Shaban \textit{et al.} \cite{shaban2017one} implements a simple network to produce weights based on the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, as the ProtoNets, that are than fused with the features extracted from the query. \cite{zhang2019sgone} uses an masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets, computing the prototypes using masked average pooling, but additionally include an \textit{alignment} loss, where prototypes are computed from the query image and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. This model uses attention modules, that receive both query features, as well as masked support images features. At last, an recurrent network is used to access information of all sample in the support set and produce the final prediction. Rakelly \textit{et al.} \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation: Guided Networks. Guided Nets use the same network to extract features of the support set and the query image. The support images are sparsed labeled and their features are masked averaged using such annotations, and further used as weights.
These works(\cite{shaban2017one, dong2018few, rakelly2018conditional, hu2019attention, zhang2019sgone, wang2019panet}) were firstly proposed to common images as seen in datasets like the Pascal VOC~\cite{pascal-voc-2012}. 

\cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs, where they construct a synthetic dataset from a single labeled image and a large unlabeled dataset using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

Although being a few-shot sparse segmentation method, we no present the Guided Nets~\cite{rakelly2018conditional} as a baseline. Even to the best of our efforts, the model did not converge with the episodic training used a single binary dataset(most of the medical datasets used). Thus, it did not seen fair to compare the Guided Nets with our approach.
% In this work we did not present the Guided Nets~\cite{rakelly2018conditional} as a baseline, although being a few-shot sparse segmentation method. There were two main problems with the method. The first, being that using pretrained DNNs from ImageNet datasets were not useful for the medical imaging used. The second, was that even to the best of our efforts, the model did not converge with the episodic training used a single binary dataset(most of the medical datasets used). Since, it did not seen fair to compare the Guided Nets with our approach.
% \todo{Justify the absence of Guided Nets as a baseline: inability to use pretrained DNNs from ImageNet and problems with episodic training on binary labels from the Meta-Dataset (did not converge to the best of our efforts).}

% FIRST VERSION
% Sparse labeling segmentation can be challenging scenario.~\citet{vernaza2017learning} tackle the sparse label scenario in an interesting manner. They propose a labeling propagation scheme using random-walk. Two networks are used, one is used in the labeling propagation and the other is an ordinary segmentation network. In training, in parallel the image is segmented by one of the networks and has the sparse labels propagated to all pixels. The train objective is that these two branches agree on the final prediction.~\citet{cciccek20163d} uses a simple approach to the sparse label scenario. The authors use an UNet architecture in 3d images of \textit{Xenopus} embryos. In this work, to train the network they reweight the importance of the voxels. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are unconsidered in computing the training loss.

% Our work is uses the approach of \cite{cciccek20163d}, to deal with sparse labels. Our methods are built upon MAML \cite{finn2017model} and ProtoNets \cite{snell2017prototypical}, thus is related to CITE. The frameworks of MAML and ProtoNets will be further detailed in the section CITE, since they are essential to our methods.

% \subsection{Few-Shot Segmentation from Sparse Labels}
% \label{sec:few_shot_sparse_seg}

% % "This is a natural extension of [24] to segmentation, but we find it is difficult to optimize for structured output, perhaps due to multi-modality or fine-tuning from pre-training. [...] In comparing feature fusion, parameter regression, and prototypes we find feature fusion is more accurate and simpler to tune. This is the inference strategy used for all of our results." \cite{rakelly2018conditional}.

% All methods referenced in Section~\ref{sec:few_shot_seg} address the problem of few-shot semantic segmentation regarding the number of labeled images used in the support set, while the methods presented in Section~\ref{sec:sparse_seg}. However, none of these methods address the scenario of few-shot learning from sparse annotations, relying on laborious dense labeling masks. Dense masks may be unfeasible or undesirable for applications that depend on annotations from specialists (e.g. biomedical imaging or remote sensing).

% \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation.

% The authors of \cite{rakelly2018conditional} use the same network to extract features of the support set and the query image, but the support features are used as weights.

==> SIBGRAPI - MetaLearning Medical/sec3_methodology.tex <==
\section{Methodology}
\label{sec:methodology}

% TODO

% \subsection{Priors for Radiological Image Segmentation}
% \label{sec:priors_seg}

% \todo{Mention that general knowledge about anatomy and general organ shapes should be initialized in biomedical segmentation models instead of random initializations.}

% \todo{Explain the recent growth in the research about inserting priors into models focusing on label-efficient (e.g. domain adaptation, self-supervision, meta-learning, knowledge distillation, etc).}

% % \todo{Introduce the idea of sparse labels being fed during meta-training and dense labels being fed during meta-test. This strategy encourages the models to predict the dense masks in the query from sparse annotations in the support set.}

% \subsection{Problem Definition}
% \label{sec:problem}

We define a segmentation task $\mathcal{S} = \{\D^{sup}, \D^{qry}, c\}$, where $\D$ is a dataset with partitions $\D^{qry}$ (or query set) and $\D^{sup}$ (or support set) such that, $\D^{qry}\cap\D^{sup}=\emptyset$. The class $c$ is the positive/foreground class for the task. A dataset $\D$ is a set of pairs $(\mathbf{x}, \mathbf{y})$, where $\mathbf{x}$ is an image and $\mathbf{y}$ is the respective semantic label, with $\mathbf{y}$ being a dense mask for images in $\D^{qry}$ and a sparsely annotated mask for the $\D^{sup}$ set. In particular, we define a few-shot segmentation task $\mathcal{F}$ as a task wherein $\D^{sup}$ has a small amount of labeled samples (e.g. 20 or less) and $\D^{qry}$ labels are absent or unknown. We refer to a few-shot task as $k$-shot when $k = |\D^{sup}|$, that is, the number of samples in its support set is $k$.
% In particular, we define a few-shot segmentation task as segmentation task $\mathcal{F}$, where the set $\D^{sup}$ have few samples (e.g. 20 or less) and the $\D^{qry}$ labels are absent or unknown. We call a few-shot task a $k$-shot task when $k = |\D^{sup}|$, i.e., the number of samples in support is $k$.

Thus, given a set of segmentation tasks $\mathcal{S} = \{\mathcal{S}_1 , \mathcal{S}_2 , \dots, \mathcal{S}_n \}$, and a target few-shot task $\mathcal{F}$, we want to segment the images from $\D^{qry}_{\mathcal{F}}$ using information from both $\mathcal{S}$ and $\D^{sup}_{\mathcal{F}}$. 
% It holds that $(\D_{\mathcal{S}_i}, c_{\mathcal{S}_i}) \cap (\D_{\mathcal{F}}, c_{\mathcal{F}}) = \emptyset$, for all $\mathcal{S}_i$, that is, no pair of image/semantic label of $\mathcal{F}$ is present in any task $\mathcal{S}_i$ in either $qry$ or $sup$ partition.
Also, it holds that no pair of image/semantic label of $\F$ is present in any task $\St_i$ in either $qry$ or $sup$ partition.

\subsection{Gradient-based Segmentation from Sparse Labels}
\label{sec:maml_seg}

As previously mentioned, we propose WeaSeL, an gradient-based approach for semantic segmentation derived from MAML~\cite{finn2017model}. A graphical representation of our method can be seen in Figure~\ref{fig:maml_seg}. 
% We propose a Meta-Learning gradient-based approach for semantic segmentation using sparse labels based on MAML. 

\renewcommand{\currprop}{0.9\columnwidth}

\begin{figure}[!t]
    \centering
    \includegraphics[clip, trim=2.2in 1.5in 2.2in 1.7in, page=1, width=\currprop]{imgs/metaseg_train.pdf}
    % \begin{subfigure}[b]{\currprop}
    %     \centering
    %     % \fbox{
    %     \includegraphics[clip, trim=2.2in 1.5in 2.2in 1.7in, page=1, width=\textwidth]{imgs/metaseg_train.pdf}
    %     % }
    %     \caption{}
    %     \label{fig:maml_seg_1}
    % \end{subfigure}
    % \begin{subfigure}[b]{\currprop}
    %     \centering
    %     % \fbox{
    %     \includegraphics[clip, trim=2.2in 1.7in 2.2in 1.7in, page=1, width=\textwidth]{imgs/metaseg_tune.pdf}
    %     % }
    %     \caption{}
    %     \label{fig:maml_seg_2}
    % \end{subfigure}
    \caption{Visualization of the proposed approach. The parameters $\theta_i$ are optimized using sparse labels from support sets. The optimal $\theta_i^*$ would be obtained if dense labels were presented in meta-training, as the ones in the query set used to compute the task outer loss. The model learns to intrinsically minimize this difference $\Delta$ between parameters, and thus fastly adapt to the few-shot task.}
    \label{fig:maml_seg}
\end{figure}

We define a meta task $\T = \{\Ls, \D^{sup}, \D^{qry}, c\}$ comprised of a loss function $\Ls$ and a pair of datasets $\D^{sup}$ and $\D^{qry}$ -- the meta-train and meta-test sets, respectively -- and a class $c$. This is an extension of the segmentation task definition from Section~\ref{sec:methodology}. We assume a distribution over tasks $p(\T)$ that our model $f_\theta$ (parametrized by $\theta$) is desired to be able to adapt to.
A description of this supervised training adaptation of MAML can be seen in Algorithm~\ref{alg:maml_gen}. 
% Given a model $f_\theta$ with trainable parameters $\theta$. In the inner loop of the algorithm, the parameters used by the model became $\theta_i$ which is initialized with the values of $\theta$. Then, $\theta_i$ is updated by one or more steps of gradient descent using, 
% $$
% \theta_i = \theta - \alpha\nabla_\theta\Ls_{\T_i}(f_\theta)
% $$
% where the step size $\alpha$ can be an fixed parameter, or meta-optimized as well.

% In the outer loop, the model's parameters $\theta$ are trained across all tasks $\T_i$ draw from $p(\T)$, by evaluating the performance of the model $f_{\theta_i}$ on that task. Thus the objective in the outer loop can be defined as,
% $$
% \min_\theta \sum_{\T_i \sim p(\T)} \Ls_{T_i} (f_{\theta_i}) = \sum_{\T_i \sim p(\T)} \Ls_{T_i} (f_{\theta - \alpha\nabla_\theta\Ls_{\T_i}(f_\theta) })
% $$
% and the parameter $\theta$ is optimized with gradient descent following
% $$\theta \leftarrow \theta - \beta\nabla_\theta \sum_{\T_i \sim p(\T)}\Ls_{\T_i}(f_{\theta_i})$$


\begin{algorithm}
    \caption{Model-Agnostic Meta Learning: Weakly Supervised}
    \label{alg:maml_gen}
    \begin{algorithmic}
        \REQUIRE $p(\T)$: distributions over tasks
        \REQUIRE $\alpha, \beta$: step size hyperparameters
        
        \STATE Randomly initialize $\theta$
        \WHILE{not done}
        \STATE Sample batch of tasks $\T_i \sim p(\T)$
        \FORALL{$\T_i$}
        \STATE Sample batch of datapoints $S_i = \{(\mathbf{x}, \mathbf{y})\}$ from $\D^{sup}_{\T_i}$
        \STATE Compute $\nabla_\theta\Ls_{\T_i}(f_\theta)$ using $S_i$ and $\Ls_{\T_i}$
        \STATE Update adapted parameters using gradient descent: $\theta_i = \theta - \alpha\nabla_\theta\Ls_{\T_i}(f_\theta)$
        \STATE Sample batch of datapoints $Q_i = \{(\mathbf{x}, \mathbf{y})\}$ from $\D^{qry}_{\T_i}$
        \ENDFOR
        \STATE Update $\theta \leftarrow \theta - \beta\nabla_\theta \sum_{\T_i \sim p(\T)}\Ls_{\T_i}(f_{\theta_i})$ using each $Q_i$ and $\Ls_{\T_i}$
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

During meta-training, the inner loss is computed using the sparse labels from samples of $\D^{sup}$, while the outer loss component takes into account the dense labels from samples of $\D^{qry}$. This strategy directly encourages the model to generate dense segmentation from the sparse labels fed on the tuning phase. Given that our problem is semantic segmentation, we define the loss function $\Ls_{\T_i}$ for all tasks $\T_i \sim p(\T)$ as the Cross-Entropy loss, ignoring the pixels with unknown labels. This is achieved by computing a weighted Cross-Entropy loss in a pixel-wise fashion, with the caveat that unknown pixels have weight $0$. When the meta-training process is finished, we fine-tune the model on the target $\mathcal{F}$ task, through a conventional supervised training on the $\D_{\mathcal{F}}^{sup}$ set, again, with a weighted cross-entropy loss.

% \subsection{Prototypical Seeds for Sparse Segmentation}
% \label{sec:prototypical_seg}

% The proposed method for semantic segmentation based on the Prototypical Networks is a straightforward adaptation of the original work~\cite{snell2017prototypical}. It uses the same premise of constructing an prototype vector to each class.

% Let $S = \{(x_1, y_1), (x_2, y_2), \dots, (x_N, y_N)\}$ be a support set, where $x_i \in \R^{H\times W \times B}$ an image with height $H$, width $W$ and $B$ channels, and $y_i \in \R^{H\times W}$ an label image with the semantic class of each pixel in $x_i$. Since $y_i$ can be sparse, the possible values of an pixel $(r,c)$ in ${y_i}$ are in the set $\{0, 1, 2, \dots, K\}$, where $K$ is the total of classes and $0$ represents the unknown class. 

% We define the prototypical vector $\mathbf{c}_k$, of an class $k$ as

% \begin{equation}\label{eq:proposed_prototype}
% \mathbf{c}_k = \frac{1}{N_k} \sum_{(x_i, y_i) \in S} f_{\theta} (x_i) \odot \mathbb{1}_k(y_i)
% \end{equation}
% where $f_{\theta}$ is our embedding function parametrized with $\theta$, $\odot$ is point-wise multiplication, and $\mathbb{1}_k(y_i) \in \{0,1\}^{H\times W}$ is a mask matrix where each value is defined as
% $$
% \mathbb{1}_k^{(r, c)}(y_i) = 
% \begin{cases}
% 1, \textnormal{ if } y_i^{(r, c)} = k \\
% 0, \textnormal{ otherwise}
% \end{cases}    
% $$
% And $N_k = \sum_{y_i} \sum_{r, c} \mathbb{1}_k^{(r, c)}(y_i)$ is the total number of pixels of the class $k$, across all the support set $S$.
% With this, our prototype vector $\mathbf{c}_k$ is the mean vector of all pixels of a class existent in the support set. 

% The inference follows~\cite{snell2017prototypical}, but applied to the pixels in the image. Formally the probability of a pixel $y^{(r,c)}$ of a query image $\mathbf{qry} \in \R^{H\times W \times B}$ belonging to a class $k$ is computed as follow:
% \begin{equation}\label{eq:proposed_proto_dist}
%     p_\theta(y^{(r, c)} = k | \mathbf{qry}) = \frac{\exp(-d(f_\theta(\mathbf{qry}), \mathbf{c}_k))}{\sum_{i} \exp(-d(f_\theta(\mathbf{qry}), \mathbf{c}_i))}
% \end{equation}
% where $d$ is the squared euclidean distance: $d(\mathbf{u}, \mathbf{v}) = ||\mathbf{u} - \mathbf{v}||^2$.

% Given equations~\ref{eq:proposed_prototype} and \ref{eq:proposed_proto_dist}, the model $f_\theta$ is trained using the negative log-probability loss $J(\theta) = - \frac{1}{N} \sum_{r, c} \log p_\theta(y^{(r,c)} = k | \mathbf{qry})$, where $N$ is the total of valid labeled pixels.

==> SIBGRAPI - MetaLearning Medical/sec4_experimental_setup.tex <==
\section{Experimental Setup}
\label{sec:experimental_setup}

\subsection{Datasets}
\label{sec:datasets}
% \todo{HUGO Revisar datasets}

As MAML requires a bundle of tasks to properly learn to learn from few-shot examples, we constructed a Meta-Dataset of radiological image segmentation tasks from publicly available datasets. More specifically, we build this Meta-Dataset using five Chest X-Ray (CXR) \cite{shiraishi2000development,jaeger2014two,pi-null-mezon,NIHwang2017chestx}, two Mammographic X-Ray (MXR) \cite{MIASsuckling1994mammographic,moreira2012inbreast} and two Dental X-Ray (DXR) \cite{PANORAMICabdi2015automatic,IVISIONsilva2018automatic} datasets. Some of these datasets contain segmentation masks for multiple organs, which were all included in the Meta-Dataset.

% In Table~\ref{tab:datasets}, we list all datasets used in the experiments. Some datasets present more than one class, but for all tasks they were binarized, that is, we define a task by selecting a dataset and one class as foreground while the remaining pixels are treated as background.
In Table~\ref{tab:datasets}, we list all datasets used in the experiments. Some datasets present more than one class, and in these cases the datasets were binarized to construct the tasks. To define a task, we select a dataset and one class as foreground. The pixels of all remaining classes are treated as background.

In order to assess the performance of WeaSeL in a certain setting, we employ a Leave-One-Task-Out methodology. That is, all tasks but the pair $(dataset, class)$ chosen as the Few-shot task ($\mathcal{F}$) are used in the Meta-Dataset, reserving $\mathcal{F}$ for the tuning/testing phase. This strategy serves to simultaneously hide the target task from the meta-training, while also allowing the experiments to evaluate the proposed algorithm and baselines in a myriad of scenarios. Such scenarios include: 1) target tasks with both large (e.g. JSRT~\cite{shiraishi2000development}) and small (e.g. Montgomery~\cite{jaeger2014two}) domain shifts compared to the ones in the meta-training set; 2) $\mathcal{F}$ tasks with image samples seen in other tasks used during meta-training, but with different target classes (e.g. JSRT \cite{shiraishi2000development}); and 3) $\mathcal{F}$ tasks with foreground class absent in all other tasks used during meta-training (e.g. JSRT heart segmentation).

\begin{table}[h!]
    \caption{List of datasets included in the meta-dataset.}
    \label{tab:datasets}
    \begin{adjustbox}{max width=\columnwidth}
        \begin{tabular}{@{}lccc@{}}
        \toprule
        \multicolumn{1}{c}{\textbf{Dataset}}                                     & \textbf{Image Type} & \textbf{\# of Images} & \textbf{Classes} \\ \midrule
        \textbf{JSRT~\citep{JSRTshiraishi2000development}} &
          X-rays &
          247 &
          \begin{tabular}[c]{@{}c@{}}Lungs, Clavicles\\ and Hearts\end{tabular} \\
        \textbf{Montgomery~\citep{jaeger2014two}}                                & X-rays              & 138                  & Lungs            \\
        \textbf{Shenzhen~\citep{jaeger2014two}}                                  & X-rays              & 662                  & Lungs            \\
        \textbf{NIH-labeled~\cite{NIHtang2019xlsor}}                             & X-rays              & 100                  & Lungs            \\
        \textbf{OpenIST~\cite{pi-null-mezon}} & X-rays              & 225                  & Lungs            \\
        \textbf{LIDC-IDRI-DRR~\citep{LIDColiveira20203d}}                        & CT-scans            & 835                  & Ribs             \\
        \textbf{MIAS~\citep{MIASsuckling1994mammographic}} &
          Mammograms &
          322 &
          \begin{tabular}[c]{@{}c@{}}Pectoral Muscle,\\ Breasts\end{tabular} \\
        \textbf{INbreast~\citep{moreira2012inbreast}} &
          Mammograms &
          410 &
          \begin{tabular}[c]{@{}c@{}}Pectoral Muscle,\\ Breasts\end{tabular} \\
        \textbf{Panoramic~\citep{PANORAMICabdi2015automatic}} &
          \begin{tabular}[c]{@{}c@{}}X-rays\end{tabular} &
          116 &
          Mandibles \\
        \textbf{UFBA-UESC~\citep{IVISIONsilva2018automatic}} &
          \begin{tabular}[c]{@{}c@{}}X-rays\end{tabular} &
          1500 &
          Teeths \\ \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

% \todo{CXRs: JSRT (lungs, clavicles and heart), Montgomery (lungs), Shenzhen (lungs), NIH-labeled (from XLSor), OpenIST}
% \renewcommand\theenumi{\textbf{\Alph{enumi}}}
% \begin{enumerate}

%     \item \textbf{JSRT Database}~\citep{JSRTshiraishi2000development}
    
%     The JSRT Database~\citep{JSRTshiraishi2000development} is a collection 247 of chest radiographs initially proposed for lung nodules identification. Masks for lungs, clavicles and hearts structures were obtained from~\cite{JSRTvan_ginneken:2006-1223}. From each anatomical structure, a task is derived.
    
%     All the images have a resolution of $2048\times2048$ and $12$ bit pixel resolution, and are gray scale.
    
%     Examples are show in Figure~\ref{fig:jsrt_example}.
    
%     \item \textbf{Montgomery Dataset}~\citep{jaeger2014two}
    
%     The Montgomery Dataset~\citep{jaeger2014two} is a set of chests X-rays collected from patients in Montgomery County, Maryland, USA. There are 138 frontal X-rays, from which 58 are from cases of Tuberculosis - the initial use case of the dataset. Alongside with information of the patient, for each X-ray, there are binary masks for segmentation of each lung.
    
%     All the X-rays are 12 bit gray scale images, and either have size $4020\times4892$ or $4892\times4020$. Examples are shown in Figure~\ref{fig:montgomery_example} . 
    
%     \item \textbf{Shenzhen Dataset}~\citep{jaeger2014two}
    
%     The Shenzhen Dataset~\citep{jaeger2014two} were publicized along with the Montogomery dataset. This set is comprised of chests X-rays collected from patients in Shenzhen, China. There are a total of 662 frontal X-rays, from which 336 are from cases of Tuberculosis. There is also binary masks for segmentation of each lung.
    
%     The size of the X-rays vary, but average a $3000\times3000$ resolution, and are gray scale. Examples are shown in Figure~\ref{fig:shenzhen_example}.
    
%     \item \textbf{NIH-labeled}~\citep{NIHwang2017chestx}
    
%     This is a subset of the original NIH-labeled dataset~\citep{NIHwang2017chestx}. The original dataset is comprised of $108,948$ frontalview X-ray images of $32,717$ unique patients, and labeled with NLP for 14 different diseases.
    
%     The subset used in this experiments will be named simply NIH-labeled or XLSor-NIH. This dataset proposed in \cite{NIHtang2019xlsor} is comprised of $100$ chest X-rays from the original NIH with manually annotated lung masks for this X-rays.
    
%     All images have a spatial resolution of $512\times512$ and are gray scale. Examples can be seen in Figure~\ref{fig:nih_example}.
    
%     \item \textbf{OpenIST Chest X-Rays}\footnote{\url{https://github.com/pi-null-mezon/OpenIST}}
    
%     The OpenIST Chest X-Rays dataset\footnote{\url{https://github.com/pi-null-mezon/OpenIST}} is a set of X-rays collected from the original webpage ChestX-rays\footnote{\url{http://www.chestx-ray.com/index.php/education/normal-cxr-module-train-your-eye#!1}}. This images were used to train medical students in recognizing a normal X-ray. There are in total $225$ chest X-ray images, with binary masks for the lungs.
    
%     The images are gray scale with 8-bit resolution and their sizes are not fixed. Examples in Figure~\ref{fig:openist_example}. 
    
    
%     \item \textbf{LIDC-IDRI-DRR dataset}~\citep{LIDColiveira20203d}
    
%     Is a dataset derived from LIDC~\citep{LIDCarmato2011lung}. This dataset is composed of flattened 2D Digitaly Reconstructed Radiographs (DRR) computed from chest CT-scans, as well as generated labels for the ribs.
    
%     All the $835$ images in the dataset are gray scale, and have size $512\times512$. Examples of the scans and labels are show in Figure~\ref{fig:lidc-idri-drr_examples}.
    
%     \todo{MXR: MIAS (pectoral, breast), INbreast (pectoral, breast) DE ONDE VEIO OS LABELS}
%     \item \textbf{MIAS database}~\citep{MIASsuckling1994mammographic}
    
%     The Mammographic Image Analysis Society (MIAS) is a research group in the UK with interest in mammograms. Their dataset is composed of $322$ digitized mammograms, grayscaled and with a resolution of $1024\times1024$. The original dataset only provides labels of location and size of nodules in the images, but we had access to label masks that segment the pectoral muscles and the breast in each image.
    
%     Example of an image and its masks are shown in Figure~\ref{fig:mias_example}
    
%     \item \textbf{INbreast database}~\citep{moreira2012inbreast}
    
%     The INbreast database is a collection of $410$ images collected from womans in the Breast Center located in the Centro Hospitalar de S. Joao [CHSJ], Porto, Portugal. From these $410$ images, only $~200$ are from MLO view, and have labeled pectoral muscles for them. We also had access to he labels of the breasts.
    
%     All images are gray level with $14$ bit resolution and their sizes are either $3328\times4084$ or $2560\times3328$, depending on the patient. Examples can be seen in Figure~\ref{fig:inbreast_example}.
    
%     \todo{DXR: Panoramix X-Ray (mandible), IVisionLab (teeth)}
%     \item \textbf{Panoramic Dental X-rays}~\citep{PANORAMICabdi2015automatic}
    
%     The Panoramic Dental X-rays dataset is a set of panoramic dental X-rays of $116$ patients, taken at Noor Medical Imaging Center, Qom, Iran. The images were mannually segment by three specialists from which a label masks for the mandibles were genereated.
    
%     All the images are gray scale and have a size of approximately $2900\times1250$ pixels. Examples of images and labels are presented im Figure~\ref{fig:panoramic_example}
    
%     \item \textbf{UFBA UESC DENTAL IMAGES Dataset}~\citep{IVISIONsilva2018automatic}
    
%     The UFBA UESC DENTAL IMAGES Dataset(or UFBA Dataset) is a composed of a series of Panoramic X-ray dental images. There is a total of $1500$ images with annotated teeth labels, with a varied cases of dental problems and/or formations. 
    
%     All the images are gray scale with dimensions of $2440\times1292$ pixels. Examples are shown in Figure~\ref{fig:ufba_example}.
% \end{enumerate}

\subsection{Architecture and Hyperparameters}
\label{sec:hyperparameters}

% \todo{Present Mini-U-Net: architecture, n\_channels in each layer, concatenation with skip connections instead of residual identity}

Due to the large computational budget of second-order optimization, we propose an architecture called miniUNet\footnote{The code for WeaSeL, including the miniUNet architecture, will be available on GitHub upon the publication of this paper.}. It is a adaptation of the usual U-Net architecture with minor changes. The network is comprised of three encoder blocks, a center block, three decoder blocks and a $1\times1$ convolutional layer that works as a pixel-classification layer.
% The network blocks configuration can be seen in table~\ref{tab:blocks}. 
Similar to the U-Net architecture skip connections between symmetric layers are present in miniUNet, with each decoder block receiving the concatenation of the last block output and its corresponding encoder output as inputs.

% \begin{table}[h!]
% \caption{Mini-U-Net Blocks descriptions}
% \label{tab:blocks}
% \setlength{\tabcolsep}{5pt}
% \begin{adjustbox}{max width=\columnwidth}
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \textbf{Block Name} & \textit{Encoder Blocks (1, 2, 3)} & \textit{Center Block} \\ \midrule
% \textbf{Layers} &
%   \begin{tabular}[c]{@{}c@{}}Conv $3\times3$\\ Bath Norm.\\ ReLU\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ MaxPool $2\times2$\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Dropout\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ T. Conv $2\times2$\end{tabular} \\
%   \midrule
% \multicolumn{1}{l}{\textbf{Input Feat./ Output Feat.}} & $C/32$, $32/64$, $64/128$         & $128/128$                  \\
% \toprule 
% \textbf{Block Name} & \textit{Decoder Blocks (3, 2)} & \textit{Decoder Block (1)} \\ \midrule
% \textbf{Layers} &
%   \begin{tabular}[c]{@{}c@{}}Dropout\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ T. Conv $2\times2$\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}Dropout\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\\ Conv $3\times3$\\ Bath Norm.\\ ReLU\end{tabular} \\
%   \midrule
% \multicolumn{1}{l}{\textbf{Input Feat./ Output Feat.}} & $256/64$, $128/32$                & $32/32$                    \\ \bottomrule
% \end{tabular}
% \end{adjustbox}
% \end{table}

% \todo{Optimizer (Adam), LR (1e-3), weight decay (5e-4), batch size (5), number of tasks in inner loop (3 -- justify with memory constraints), loss (with ignore\_index for the unlabeled pixels)}


% wAs previously mentioned, the loss ignored unlabeled pixels in both WeaSeL and baselines. 



\subsection{Evaluation Protocol and Metrics}
\label{sec:protocol}

We use a 5-fold cross validation protocol in the experiments, wherein datasets were divided in training and validation sets for each fold. Support sets are obtained from the training partition, while the query sets are the entire validation partition. All images and labels are resized to $128\times128$ prior to being fed to the models in order to standardize the input size and minimize the memory footprint of MAML on high-dimensional outputs. The metric within a fold is computed for all images in the query set according to the dense labels, resulting in the final values reported in Section~\ref{sec:results}, which are computed by averaging the performance across all folds. The metric used is the Jaccard score (or Intersection over Union -- IoU) of the validation images, a common metric for semantic segmentation.

% This measure the similarity between the ground truth and the segmentation of the model. Given two sets $A$ and $B$ is computed as follow:
% $$
% J(A, B) = \frac{|A\cap B|}{|A\cup B|}
% $$

% \todo{Preprocessing: resize to 128x128, types of sparsity (points, contours, grid, etc), density of labels (variation in n\_points, variation in contour density, space between grid pixels, etc)}

% \todo{5-Fold (avg +/- std), mention confidence intervals}

% \todo{Jaccard}

\subsection{Baselines and Sparsity Modalities}
\label{sec:baselines}

We use two baselines: 1) \textit{From Scratch} training on the sparse labels; and 2) \textit{Fine-Tuning} a pretrained model from a source dataset with \textit{dense} labels. During the meta-training phase of WeaSeL, the tuning phase of \textit{Fine-Tuning}, and \textit{From Scratch} training, the sparse labels are simulated for each sample from their the dense mask.

Although being a few-shot sparse segmentation method, we do not present the Guided Nets \cite{rakelly2018conditional} as a baseline. Even to the best of our efforts, the episodic training of the original model was not able to converge to a usable model with the same medical Meta-Dataset used by WeaSeL. Thus, it did not seem fair to compare the Guided Nets to our approach.
% \begin{itemize}
%     \item \textbf{Scratch}: We perform a simple supervised train on the Mini-Unet architecture with the Few-shot task support set ($\D^{sup}_{\mathcal{F}}$).
%     \item \textbf{Fine-tuning}: We choose one task $\mathcal{S}_i$ and perform a simple supervised train with the $\D_{\mathcal{S}_i}^{sup}$ and then fine-tune (a supervised train) on $\D^{sup}_{\mathcal{F}}$.
%     % \item \textbf{Guided}~\cite{rakelly2018conditional}: We use an adaptation of the code provided by the authors\footnote{\url{https://github.com/shelhamer/revolver}}, with the late fusion approach. Its is similar to the \textit{fine-tuning} baseline. We choose one task $\mathcal{S}_i$ and train the model in a similar manner to the authors: we sample a query image from $\D_{\mathcal{S}_i}^{qry}$ and a sparse labeled support image from $\D_{\mathcal{S}_i}^{sup}$, and use this pair for training, in each iteration. In evaluation, each image from $\D_{\mathcal{F}}^{qry}$ uses the whole $\D_{\mathcal{F}}^{sup}$ set to extract their guides.
% \end{itemize}
% \todo{Mention baselines: shallow, from scratch (vanilla DL), fine-tuning from related source data (DA), Guided Nets (pretraining + late fusion).}

% \subsection{Types of Sparse Masks}
% \label{sec:types_masks}

We evaluate two types of sparse labeling, namely, \textit{points} and \textit{grid}, as well as their comparison to the performance of the models trained on the full masks. The \textit{points} labels are a selection from pixels of the image, where the annotator alternately chooses pixels from the foreground and background. In the \textit{grid} labeling the annotator receives a pre-selected group of pixels and change the class of the ones they consider positive. These pixels are disposed in a grid manner in the image. A visualization of these styles are presented in Figure~\ref{fig:sparse_modalities}.

We simulate this two types of annotations from ground truth labels. For the \textit{points} labels, given a parameter $n$, we randomly select $n$ pixels from the foreground class, and $n$ from the background. For the \textit{grid} annotation, given a parameter $s$, we choose pixels spaced, horizontally and vertically, by $s$, starting from a random distance in the range $(0-s)$ from the upper-left corner. For a consistent evaluation, a random seed for the Few-Shot $\F$ task labels is fixed for each image, ensuring that all methods use the same sparse labels for the fine-tuning process. In experiments, we vary the parameters $n$ and $s$, and analyze the impact of the sparsity of the labels.

\renewcommand{\currprop}{0.75\columnwidth}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\currprop]{imgs/sparse_modalities.pdf}
    \caption{Example of the evaluated type of annotations. \textbf{Top Row}: the ground truth labels of all pixels. \textbf{Middle Row}: the \textit{points} annotation, $n$(5) pixels of background/foreground are labeled. \textbf{Bottom Row}: the \textit{grid} annotation, pixels spaced by $s$(20) are selected and properly labeled.}
    \label{fig:sparse_modalities}
\end{figure}


% \todo{Describe points, contours, grid, regions and full labelings.}

==> SIBGRAPI - MetaLearning Medical/sec5_results.tex <==
\section{Results}
\label{sec:results}
% \todo{HUGO: Graficos ou tabelas? R: Gráficos ;)}

% \renewcommand{\currprop}{0.7\columnwidth}

\begin{figure}[!t]
    \centering
    % \fbox{
    \centering
    \subfloat[JSRT Lungs] {
        \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/jsrt_lungs.pdf}
        \label{fig:results_jsrt_lungs}
    }
    \hfill
    \subfloat[OpenIST Lungs] {
        \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/openist_lungs.pdf}
        \label{fig:results_openist_lungs}
    }
    % \includegraphics[clip, trim=0.0in 0.0in 0.9in 0.0in, page=1, width=\currprop]{imgs/results_jsrt_lungs.pdf}
    % % }
    \caption{Jaccard results for lung segmentation in two target datasets: JSRT (a) and OpenIST (b). Solid lines indicate the performance of the methods using sparse label (\textit{Points} on the top and \textit{Grid} on the bottom), while the dashed line presents the performance of the methods trained with the dense masks.}
    \label{fig:results_lungs}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     % \fbox{
%     \includegraphics[clip, trim=0.0in 0.0in 0.9in 0.0in, page=1, width=\currprop]{imgs/results_openist_lungs.pdf}
%     % }
%     \caption{\todo{Caption...}}
%     \label{fig:results_openist_lungs}
% \end{figure}

\begin{figure}[!t]
    \centering
    % \fbox{
    \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/jsrt_heart.pdf}
    % \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/jsrt_heart.pdf}
    % }
    \caption{Jaccard results for heart segmentation in JSRT dataset.}
    \label{fig:results_jsrt_heart}
\end{figure}

% \begin{figure}[!t]
%     \centering
%     % \fbox{
%     \includegraphics[clip, trim=0.0in 0.0in 0.9in 0.0in, page=1, width=\currprop]{imgs/results_jsrt_clavicles.pdf}
%     % }
%     \caption{\todo{Caption...}}
%     \label{fig:results_jsrt_clavicles}
% \end{figure}

We perform experiments to access the performance of WeaSeL in all CXR datasets. That is, we evaluate the Few-shot task segmentation of lungs in all five datasets, and hearts and clavicles segmentation in the JSRT dataset. 
For brevity, we include only a subset of the results.
% , as the remainder will be presented in Supplementary Material, which also include visual results of our method in the evaluated tasks.

In Figure~\ref{fig:results_lungs} we see the results of experiments in the lungs class. The results of Montgomery and Shenzhen datasets are similar to the OpenIST, thus we only present the later. WeaSeL shows better metrics than the \textit{From Scratch} baseline in all cases. As expected, increasing the amount of annotated pixels (e.g. by increasing $n$, or decreasing the grid spacing $s$), as well as having more training samples (larger $k$-shots), have a direct impact in IoU. For JSRT (Figure~\ref{fig:results_jsrt_lungs}), WeaSeL yields better performance than \textit{Fine-Tuning} from all datasets, in contrast with OpenIST (Figure~\ref{fig:results_openist_lungs}) where the source dataset was decisive in the performance of \textit{Fine-Tuning}. The networks pretrained on JSRT achieved performances lower than WeaSeL, while the pretraining from Shenzhen or Montgomery yielded better results than our approach. This discrepancy can be explained by the different domains, as the JSRT dataset is the most singular within the five CXR datasets -- that is, the domain shift between JSRT and the other datasets is larger than the shift between the other four. It should be noticed that real-world scenarios may not allow for a fair evaluation of the domain shift between the source and target datasets, making WeaSeL the safer choice in this case. %This difference makes fine-tunning from one of the similar datasets an efficient method for few-shot, since the data from these datasets have a similar distribution, while MAML is better to generalize from more diverse tasks.

In Figure~\ref{fig:results_jsrt_heart} we see the results for the heart class in JSRT. This, and the clavicles class, are only present in the JSRT dataset. 
% The tasks chosen for the \textit{Fine-Tuning} baselines were the pairs of JSRT dataset and one of the other classes as target.
Since these classes are only present in JSRT, for the \textit{Fine-Tuning} baselines we choose the pairs of JSRT dataset and one of the remaining classes as source tasks (e.g., for hearts we use the pairs $(JSRT, lungs)$, and $(JSRT, clavicles)$).
Again, the \textit{From Scratch} baseline is the worst performer, with the WeaSeL being the superior in most scenarios. The clavicles, display a similar tendency, although their IoU score, in majority of the cases, is lower than the heart class scores.

\begin{figure}[!t]
    \centering
    % \fbox{
    \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/inputs_jsrt_lungs.pdf}
    % \includegraphics[clip, trim=0.0in 0.0in 0.0in 0.0in, page=1, width=\columnwidth]{imgs/jsrt_heart.pdf}
    % }
    \caption{Jaccard results of the WeaSeL method in the JSRT Lungs task by the average number of inputs.}
    \label{fig:inputs_jsrt_lungs}
\end{figure}

% As we can see in both experiments, the performance of the \textit{grid} annotation is higher than the \textit{points} annotation. This was expected, since, even in the larger spacing scenario($s=20$) the number of annotated pixels is greater than the the $2n$ pixels in any \textit{points} labeling case. Even with a likely class imbalance in the \textit{grid} scenario --- the foreground is usually smaller than the background, and with a fixed grid will probably have fewer labeled pixels ---, the simple presence of more data increases the metric score for this type of annotation.

As seen in both experiments, the performance of the \textit{grid} annotation is higher than the \textit{points} annotation, in virtually all cases. In order to assess the efficiency of this annotations we constructed the graph in Figure~\ref{fig:inputs_jsrt_lungs}. The \textit{x} axis represents the average number of inputs per image, and was computed considering each positive labeled pixel in an image as an user input, and then average across all images. In the figure, we confirm the overall better performance of the \textit{grid} annotation, and a better efficiency as the score of the method with the same number of inputs is higher using this annotation over the \textit{point} annotation. One explanation is that even in the larger spacing scenario($s=20$) the number of annotated pixels is greater than the the $2n$ pixels in any \textit{points} labeling case. Thus, even with a likely class imbalance in the \textit{grid} scenario --- the foreground objects is usually smaller than the background, and with a fixed grid will probably have fewer labeled pixels ---, the simple presence of more data increases the metric score for this type of annotation.

% Although, in general having a worse performance than with dense labeling, the sparse annotations have 
% competitive results considering the number of labeled pixels.
Sparse annotation show competitive results with dense labels, given the much smaller labeled data.
The case with most labeled data is the \textit{grid} annotation with $s=20$, that have approximately $~2\%$ of annotated pixels. In some cases, the methods using sparse labels are equivalent to using dense labels ground truths, specially with the \textit{grid} annotation. In the lungs segmentation in the OpenIST (and Montgomery/Shenzhen) dataset (Figure~\ref{fig:results_openist_lungs}), the \textit{Fine-tuning} baselines from similar datasets seem indifferent to sparse or dense labels. As aforementioned, the small domain shifts between these datasets and the pretraining with dense labels explain this results.

\section{Qualitative Analysis}
\label{sec:qualitative}

In Figures~\ref{fig:jsrt_lungs_visual}-\ref{fig:jsrt_heart_visual} we show visual segmentation examples of WeaSeL on three tasks: JSRT Lungs, OpenIST Lungs and JSRT Heart, respectively. In each example, lines represent the number of shots in the experiment, while columns vary the sparsity parameters: $n$ for points (first four columns) and $s$ for grids (last four columns). These sparsity scenarios were used to simulate the sparse labels of the support set on the target few-shot task.

As one can observe in these visual results, increasing the annotation density -- that is, increasing the number of points $n$ or using a smaller spacing $s$ -- yields a larger improvement in the predictions than increasing the number of labeled images; that is, the number of shots. Even the 1-shot scenario achieved acceptable results for the lung tasks (Figures~\ref{fig:jsrt_lungs_visual},~\ref{fig:openist_lungs_visual}) when given a sufficient number of labeled pixels, e.g. at least 20 labeled pixels for each class.
For heart segmentation (Figure~\ref{fig:jsrt_heart_visual}), we observe a great difference between the points and grid annotations. Since this is a unique task -- i.e. the only task in the meta-dataset with \textit{heart} as a target class, which is only present in the JSRT dataset -- the model requires more support samples/labels to adapt to this task. This requirement is not fully achieved by the points annotation with one and five shots, but is obtained by less sparse grid annotations in all observed number of shots. Again, the total number of labeled pixels in the grid annotation seems to compensate the lack of images for training.

It is clear that having a larger number of annotated images impacts the final results, especially for harder, or more distinct, datasets or tasks as is the case of JSRT. Consequently, a middle ground in relation to the number of images and the sparsity of annotations seems to be a good compromise to achieve reasonable results with limited human intervention. That is, annotating five or more images with at least five pixels labeled per class can lead to good results with a very low labeling burden. However, if the target task is truly few-shot, increasing the number of samples in the support set may be costly or even impossible. In this case, one can instead increase the per sample label density.


\newcommand\cincludegraphics[2][]{\raisebox{-0.1\height}{\includegraphics[#1]{#2}}}
\newcommand\exImages{0.15}


% \todo{Comentar a variação do número de points vs. número de shots. Vale mais a pena anotar mais samples esparsamente ou menos samples mais densamente? Em que ponto a segmentação fica visualmente "aceitável" de acordo com a forma do órgão?}

% \begin{table*}[h!]
% \resizebox{\textwidth}{!}{
    % \begin{tabular}{cllllllll}
    % \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Image}} & \multicolumn{4}{c}{\textbf{Ground Truth}} \\
    % \multicolumn{1}{l}{} & \multicolumn{4}{c}{
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/JPCLN060.png}} & \multicolumn{4}{c}{
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/gt_JPCLN060.png}} \\
    % \multicolumn{9}{l}{} \\
    % \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Points}} & \multicolumn{4}{c}{\textbf{Grid}} \\
    % \textbf{Shots} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{5}} & \multicolumn{1}{c}{\textbf{10}} & \multicolumn{1}{c}{\textbf{20}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{12}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{20}} \\
    % \textbf{1} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_1_points_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_5_points_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_10_points_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_20_points_JPCLN060.png}&
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_8_grid_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_12_grid_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_16_grid_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_20_grid_JPCLN060.png}\\
    % \textbf{5} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_1_points_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_5_points_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_10_points_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_20_points_JPCLN060.png}&
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_8_grid_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_12_grid_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_16_grid_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_20_grid_JPCLN060.png}\\
    % \textbf{10} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_1_points_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_5_points_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_10_points_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_20_points_JPCLN060.png}&
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_8_grid_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_12_grid_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_16_grid_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_20_grid_JPCLN060.png}\\
    % \textbf{20} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_1_points_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_5_points_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_10_points_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_20_points_JPCLN060.png}&
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_8_grid_JPCLN060.png} &
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_12_grid_JPCLN060.png} & 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_16_grid_JPCLN060.png}& 
    % \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_20_grid_JPCLN060.png}
    % \end{tabular}
    % }
    % \captionof{figure}{Visual segmentation examples for JSRT Lungs.}
% \end{table*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{imgs/results_qualitative_jsrt_lungs.pdf}
    \caption{Visual segmentation examples for the JSRT Lungs task.}
    \label{fig:jsrt_lungs_visual}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{imgs/results_qualitative_openist_lungs.pdf}
    \caption{Visual segmentation examples for the OpenIST Lungs task.}
    \label{fig:openist_lungs_visual}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \includegraphics[width=0.85\textwidth]{imgs/results_qualitative_jsrt_heart.pdf}
    \caption{Visual segmentation examples for the JSRT Heart task.}
    \label{fig:jsrt_heart_visual}
\end{figure*}

% \begin{table*}[h!]

% \resizebox{\textwidth}{!}{
% \begin{tabular}{cllllllll}
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Image}} & \multicolumn{4}{c}{\textbf{Ground Truth}} \\
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/JPCNN038.png}} & \multicolumn{4}{c}{
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/gt_JPCNN038.png}} \\
% \multicolumn{9}{l}{} \\
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Points}} & \multicolumn{4}{c}{\textbf{Grid}} \\
% \textbf{Shots} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{5}} & \multicolumn{1}{c}{\textbf{10}} & \multicolumn{1}{c}{\textbf{20}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{12}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{20}} \\
% \textbf{1} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_1_points_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_5_points_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_10_points_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_20_points_JPCNN038.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_8_grid_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_12_grid_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_16_grid_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/1_shot_20_grid_JPCNN038.png}\\
% \textbf{5} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_1_points_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_5_points_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_10_points_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_20_points_JPCNN038.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_8_grid_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_12_grid_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_16_grid_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/5_shot_20_grid_JPCNN038.png}\\
% \textbf{10} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_1_points_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_5_points_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_10_points_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_20_points_JPCNN038.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_8_grid_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_12_grid_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_16_grid_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/10_shot_20_grid_JPCNN038.png}\\
% \textbf{20} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_1_points_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_5_points_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_10_points_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_20_points_JPCNN038.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_8_grid_JPCNN038.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_12_grid_JPCNN038.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_16_grid_JPCNN038.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/jsrt_lungs_visuals/20_shot_20_grid_JPCNN038.png}
% \end{tabular}
% }
% \captionof{figure}{Visual segmentation examples from JSRT Lungs task.}
% \label{tab:jsrt_lungs_visual2}
% \end{table*}

% \begin{table*}[h!]

% \resizebox{\textwidth}{!}{
% \begin{tabular}{cllllllll}
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Image}} & \multicolumn{4}{c}{\textbf{Ground Truth}} \\
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/131-140-500-500-100.png}} & \multicolumn{4}{c}{
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/gt_131-140-500-500-100.png}} \\
% \multicolumn{9}{l}{} \\
% \multicolumn{1}{l}{} & \multicolumn{4}{c}{\textbf{Points}} & \multicolumn{4}{c}{\textbf{Grid}} \\
% \textbf{Shots} & \multicolumn{1}{c}{\textbf{1}} & \multicolumn{1}{c}{\textbf{5}} & \multicolumn{1}{c}{\textbf{10}} & \multicolumn{1}{c}{\textbf{20}} & \multicolumn{1}{c}{\textbf{8}} & \multicolumn{1}{c}{\textbf{12}} & \multicolumn{1}{c}{\textbf{16}} & \multicolumn{1}{c}{\textbf{20}} \\
% \textbf{1} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_1_points_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_5_points_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_10_points_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_20_points_131-140-500-500-100.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_8_grid_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_12_grid_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_16_grid_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/1_shot_20_grid_131-140-500-500-100.png}\\
% \textbf{5} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_1_points_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_5_points_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_10_points_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_20_points_131-140-500-500-100.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_8_grid_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_12_grid_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_16_grid_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/5_shot_20_grid_131-140-500-500-100.png}\\
% \textbf{10} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_1_points_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_5_points_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_10_points_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_20_points_131-140-500-500-100.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_8_grid_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_12_grid_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_16_grid_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/10_shot_20_grid_131-140-500-500-100.png}\\
% \textbf{20} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_1_points_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_5_points_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_10_points_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_20_points_131-140-500-500-100.png}&
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_8_grid_131-140-500-500-100.png} &
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_12_grid_131-140-500-500-100.png} & 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_16_grid_131-140-500-500-100.png}& 
% \cincludegraphics[width=\exImages\textwidth]{imgs/openist_lungs_visuals/20_shot_20_grid_131-140-500-500-100.png}
% \end{tabular}
% }
% \captionof{figure}{Visual segmentation examples for OpenIST Lungs.}
% \label{tab:openist_lungs_visual}
% \end{table*}

==> SIBGRAPI - MetaLearning Medical/sec6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We evaluated WeaSeL, our proposed adaptation of MAML, in multiple few-shot segmentation tasks with sparse labels. WeaSeL showed to be a viable solution to most tasks, and a suitable option when there are very discrepant target and source tasks. Since in real-world scenarios is difficult to access the domain shift between the datasets, WeaSeL seems to be the safer choice in these cases. The method have some limitations, like the cost of computing second-derivatives in the outer loop. This limited the size of training images to $128\times128$, which can hinder task with small target objects (e.g. clavicles). 

Future works include the use of approximations to the second derivative and how this affects the performance, as well as analyzing different types of sparse labels annotations also in 3D volumes. Additionally, we intend to adapt other first- and second-order Meta-Learning methods for sparsely labeled semantic segmentation.

% For future works there are two principal points we want to work, that are: 1) different types of sparse labels annotations; 2) adapt other Meta-Learning algorithms for sparse segmentation.
% One future investigation, is the impact of using first-order approximation of the second derivatives, and how this will affect the segmentation, but can allow the use of larger images in training.
% \todo{Future works: 1) labeling configurations; 2) adapting other Meta-Learning algorithms for sparse segmentation.}

==> sec2_related_old.tex <==
\section{Related Work}
\label{sec:related}

% FIRST VERSION
% Automatic segmentation of medical images has been studied for many years. Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. \citet{nie2016fully} uses a Fully Convolutional Neural Network(FCN)~\cite{long2015fully} to segment brain tissue in infants. The authors propose an architecture to segment Magnetic Resonance imaging (MRI) of brains in in 4 categories: white matter (WM), gray matter (GM), and cerebrospinal fluid (CSF) and background. \citet{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net. They use this network to perform multiple organs segmentation in 3d abdominal Computed tomography(CT) imaging. In~\cite{gordienko2017} the authors studies lungs segmentation. They use an U-Net \cite{ronneberger2015u} architecture to segment lungs from the background in XRay images from the JSRT dataset~\cite{shiraishi2000development}. In a similar procedure,~\cite{skourt2018lung} also performs lung segmentation. In this work, they train an U-Net in the Lung Image Database Consortium image collection (LIDC-IDRI)~\cite{lidc-idri}.

Automatic and semi-automatic segmentation of medical images has been studied for decades, as such methods can considerably alleviate the burden of physicians in labeling these data \cite{ronneberger2015u}. Medical image segmentation from sparse labels can be especially useful, as biomedical images often have a small number of labeled samples due to data privacy restrictions and the lack of specialists for annotating the samples. Additionally, Few-Shot learning has attracted considerable attention over the last years, mainly due to recent advances in Deep Learning for Self-Supervised learning \cite{goyal2019scaling} and Meta-Learning \cite{snell2017prototypical,finn2017model}. However, the intersection of Few-Shot learning and medical image segmentation from sparse labels has proven to be quite a challenging task, with very few methods being described in the literature \cite{wang2018interactive}.
% Recently, Deep Learning techniques, especifically using CNNs became the state-of-the-art. 
% The works \cite{nie2016fully,gibson2018automatic,gordienko2017,skourt2018lung} use a variation of a CNN to segment various type of medical images. In \cite{gordienko2017,skourt2018lung} they use an U-Net~\cite{ronneberger2015u} architecture, while \cite{nie2016fully} uses an Fully Convolutional Network(FCN)~\cite{long2015fully}, and \cite{gibson2018automatic} proposes a new convolutional architecture called DenseV-Net, similar to an U-Net. 
% Both \cite{gordienko2017,skourt2018lung} perform lung segmentation in different types of images. \cite{gordienko2017} work with XRay images from JSRT dataset~\cite{shiraishi2000development} and \cite{skourt2018lung} Computed Tomography(CT) images from LIDC-IDRI~\cite{lidc-idri}.~\cite{gibson2018automatic} also use CT images, but from abdominal region, while \cite{nie2016fully} focus on Magnetic Resonance Imaging(MRI) of infant brains. 

% \todo{Mention the survey on medical image segmentation with noisy/sparse labels by \cite{tajbakhsh2020embracing}. Use taxonomy to define our methodology. Provide a table in the related work organizing the referenced papers using the taxonomy.}

% The survey of Tajbakhsh et. al~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation. This survey includes a section for segmentation with noisy/sparse labels. The methods for sparse label can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse, bai2018recurrent, cai2018accurate, can2018learning, matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, i.e.~\cite{cciccek20163d, silvestri2018stereology, bokhorst2018learning, zhu2019pick} --- \cite{cciccek20163d, bokhorst2018learning} using a weighted loss, \cite{silvestri2018stereology} implies the use of padding in the sparse labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based of the sparse annotation.

% The innate nature of semantic segmentation makes sparse labeling a challenging scenario.~\cite{vernaza2017learning} approach this case with a label propagation scheme. The authors propose an two branch pipeline, one of an ordinary segmentation network and the other a label propagation using random-walk. During training the two branches are expected to agree on the pixel classification.~\cite{cciccek20163d} proposes a much simpler method to sparse label scenarios. Working with 3D images of \textit{Xenopus} embryos with only a few annotated voxels, the authors reweight the importance of diferent classes in the objective function. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are ignored when computing the training loss.

% \subsection{Meta-Learning for Few-Shot Scenarios}
% \label{sec:meta_learning}

% In recent years, many works had focused on Few-Shot scenarios, specifically for the classification task. The works \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} can be seen as a form of Metric Learning approach, were the models learn embedding functions to a space different of the input (REVISION NEEDED). \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses the support set - the set of few labeled images - to guide its transformation, than the model uses a weighted average to predict the class probability of the query image (i.e. the image of interest, in this task, an image to be classified). \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets). This model tries to learn em embedding function that computes \textit{prototypes} to a class (i.e. a $d$-dimensional vector that represents a class). When predicting a query image class, the model computes its prototype and compares with the class prototypes produced by the support set, being the closest one assigned as the predicted label. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs). Their model, learns to create an $d$-dimensional subspace from the support set, for each class. A query image is than embedded to this space and the distance of their projection to each subspace is computed. The subspace with the smaller projection distance is chosen as the class of the query.

% There have been an increasingly use of meta-learning to Few-Shot scenarios, primarily classification. Generally, these methods can be divided in metric learning and optimization approaches. The former focusing on models learning embedding functions, and computing distances in the embedding spaces. The later focusing in new methods to direct optimize models in this data regime.

% \cite{vinyals2016matching,snell2017prototypical,Simon_2020_CVPR} are examples of Metric Learning approaches. \cite{vinyals2016matching} proposes the Matching Networks, an attention based model that uses a small set of images to guide its transformation. \cite{snell2017prototypical} proposes the Prototypical Networks (ProtoNets), a model that tries to learn em embedding function that computes \textit{prototypes} to a class (i.e. a $d$-dimensional vector that represents a class) and uses these distance to these prototypes for inference. In \cite{Simon_2020_CVPR} the authors presents the Deep Subspace Networks (DSNs), a model that learns to create an $d$-dimensional subspace from the support set, for each class, and the projection distance to these subspaces are used for class prediction. 

% A different strategy can be seen in the works \cite{finn2017model, raghu2019rapid, yoon2018bayesian, finn2018probabilistic}, that can be described as Gradient-Based, that is algorithms that proposes novel gradient optimizations to train models in this data regime (REVISION NEEDED). In \cite{finn2017model} the authors proposed the MAML framework. In this framework they use multiple tasks (an small data sample for train/test with an loss function). They train the model to generalize well to these tasks. 
% There is an \textit{outer} an \textit{inner} loop in the training process. The outer loop, an global parameter $\Theta$ is optimized to provide good initialization parameters for specific tasks. In the inner loop, the model takes the global $\Theta$ and create a $\Theta_i$ specific to each task sampled in that outer loop iteration, producing a task specific loss based of them. The summation of these losses is than used to compute the gradients to the global $\Theta$.
% % There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
% The work~\cite{raghu2019rapid} is an modification of the MAML~\cite{finn2017model} model. The novel proposed by \cite{raghu2019rapid} is that in the \textit{inner} loop of MAML, instead of updating all the $\Theta$ parameters, they only update the parameters related to the network head (the components of the network that are correspondent to an classifier, in this case). With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) \cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop. \cite{finn2018probabilistic} presents an probabilistic version of MAML. The $\Theta$ parameters are not the weights of an network, but instead they define a distribution over such weights. During training, in the inner loop, they use information over the test set of a task to sample the weights that will be updated for a task. The outer loop loss also include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

The works \cite{finn2017model, raghu2019rapid, yoon2018bayesian, finn2018probabilistic}, can be seen as Optimization/Gradient-Based approaches. Finn \textit{et al.} \cite{finn2017model} propose the Model-Agnostic Meta-Learning (MAML) framework, based on the trend of Optimization/Gradient-based approaches. In this framework they use multiple tasks (an small data sample for train/test with an loss function) in training to create a general model. 
There are two nested loops(\textit{outer} an \textit{inner}) in the training process. In the inner loop the model is optimized to minimize the loss of a task, while the outer the model parameters are optimized to be generally usable for all tasks. 
% There is a global parameter $\Theta$, and a parameter $\Theta_i$ computed for each task from the optimization of $\Theta$ in that task. Than the global $\Theta$ is optimized from an summation of the tasks specific losses.
The work~\cite{raghu2019rapid} is an modification of the MAML algorithm, which consists in only update the parameters related to the network head (the components of the network that are equivalent to a classifier, in this case) within the \textit{inner} loop, instead of all the model parameters.
% With these change, the network converge to parameters that are reusable to multiple tasks, and reduce the computational cost of training. (REVISABLE) 
\cite{yoon2018bayesian} introduces BMAML, an bayesian emsemble method. They are similar to the MAML, with the outer and inner loops. However, in the inner loop they use of SVGD~\cite{liu2016stein} to update their parameters that are use to compute the loss of the outer loop.
\cite{finn2018probabilistic} presents an probabilistic version of MAML. The parameters of the model define a distribution over such weights of a network. In the outer loop, they include an additional term of Kullback-Leibler Divergence between the distributions in regards to train and test sets. 

% \subsection{Semantic Segmentation from Sparse Labels}
% \label{sec:sparse_seg}

% \todo{Mention \cite{lin2016scribblesup} as a precursor in the area. Does not rely on meta-learning, modern DA, etc. Simply works with a standard FCN, label propagation and pre-training.}

One of the first works to use sparse labels for semantic segmentation is \cite{lin2016scribblesup}, where they use a scheme of label propagation from the scribble annotations in conjunction with a FCN for segmentation. \cite{wang2018interactive} uses a principle similar to \cite{lin2016scribblesup}, but applied to biomedical images. The difference is that the model is trained on full annotations, and then the model iteratively refines their segmentation for an image, possibly using scribbles provided by the user interactively.  

% \todo{Mention the paper by \cite{wang2018interactive} about interactive sparse-labeled segmentation for biomedical images.}

Moreover, the survey of Tajbakhsh \textit{et. al}~\cite{tajbakhsh2020embracing} reviews a collection of deep learning solutions on medical image segmentation, which includes a section for segmentation with noisy/sparse labels. The methods reviewed can be summarized in a selective loss with or without mask completion. That is, all methods use a loss function that ignore unlabeled pixels/voxels, but works like~\cite{zhang2019sparse,bai2018recurrent,cai2018accurate,can2018learning,matuszewski2018minimal} use some technique to augment the sparse annotations to resemble complete masks, while others do not try to reconstruct a mask, e.g.~\cite{cciccek20163d,silvestri2018stereology,bokhorst2018learning,zhu2019pick} --- \cite{cciccek20163d,bokhorst2018learning} using a weighted loss, Silvestri \textit{et al.} \cite{silvestri2018stereology} implies the use of padding of labels, and \cite{zhu2019pick} uses a quality model to ensure a good segmentation based on sparse annotations.

\subsection{Few-Shot Semantic Segmentation}
\label{sec:few_shot_seg}

% FIRST VERSION
% Few-shot semantic segmentation is a field that only recently started to be explored.~\citet{shaban2017one} proposes a method to few-shot segmentation. A two-branch network is used, one branch is a usual segmentation network, such as FCN, the other branch receives an support set of images and produce weights. This weights are  used in the other branch to perform the final segmentation.~\citet{dong2018few} introduces an architecture for few-shot semantic segmentation based on the prototypical networks~\cite{snell2017prototypical}, that were originally proposed for classification. Their framework is divided in two network. One is used to produce the prototypes for each class in the query image using the support set. The second produces a feature map from the query image, this map is weighted using the prototypes. The weighted feature map is than used to produce the final segmentation.~\citet{rakelly2018conditional} is similar to \cite{shaban2017one}. The difference is that in \cite{rakelly2018conditional} the authors use the same network to extract the features from the query and support images. The features of the support images are further use to "guide" the segmentation of the query image, that is, these features are aggregated to the ones of the query image, and then processed to generate the segmentation. The works~\cite{dong2018few, shaban2017one, rakelly2018conditional} were firstly proposed to usual photographs. \citet{zhao2019data} tackled one-shot segmentation in brain MRIs. The authors proposed a framework where they use CNN to learn transformations that can be used to data augment their dataset. With the trained networks and a single annotated image, they synthesize a dataset from unlabeled brain MRIs. This dataset is then used to train a network in a supervised fashion.

% Few-shot semantic segmentation became a relevant topic only recently. Works like \cite{shaban2017one, dong2018few, hu2019attention, zhang2019sgone, wang2019panet} present some approaches to use the support set to segment the query image. In \cite{shaban2017one} implements a simple network for the extraction of the weights from the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, that are than fused with the features extracted from the query, thus being an adaptation of the Prototypical Networks~\cite{snell2017prototypical}. \cite{zhang2019sgone} uses an masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets. The authors compute the prototypes using masked average pooling, but additionally an \textit{alignment} loss is used, where the query image is used to produce the prototypes and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. This model uses attention modules, that receive both query features, as well as masked support images features. At last, an recurrent network is used to access information of all sample in the support set and produce the final prediction. These works(\cite{shaban2017one, dong2018few, rakelly2018conditional, hu2019attention, zhang2019sgone, wang2019panet}) were firstly proposed to usual photographs as seen in datasets like the Pascal VOC~\cite{pascal-voc-2012}. \cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs. The authors use a single labeled example and a large set of unlabeled images to construct a synthetic dataset, using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

Few-shot semantic segmentation became a relevant topic only recently. Works like \cite{shaban2017one, dong2018few, hu2019attention, zhang2019sgone, wang2019panet} present some approaches to use the \textit{support set} --- the small set of labeled images --- to segment a query image. Shaban \textit{et al.} \cite{shaban2017one} implements a simple network to produce weights based on the support set, that are used as parameters of a logistic regression prediction. \cite{dong2018few} creates a network to produce prototypes of each class, as the ProtoNets, that are than fused with the features extracted from the query. \cite{zhang2019sgone} uses an masked average pooling to construct class representative vectors, that are further used to compute a similarity map - using cosine distance -, that are fused with features of query image. \cite{wang2019panet} proposes an adaptation of ProtoNets, computing the prototypes using masked average pooling, but additionally include an \textit{alignment} loss, where prototypes are computed from the query image and the support set is the segmentation target. In~\cite{hu2019attention}, the authors introduce an attention-based model. This model uses attention modules, that receive both query features, as well as masked support images features. At last, an recurrent network is used to access information of all sample in the support set and produce the final prediction. Rakelly \textit{et al.} \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation: Guided Networks. Guided Nets use the same network to extract features of the support set and the query image. The support images are sparsed labeled and their features are masked averaged using such annotations, and further used as weights.
These works(\cite{shaban2017one, dong2018few, rakelly2018conditional, hu2019attention, zhang2019sgone, wang2019panet}) were firstly proposed to common images as seen in datasets like the Pascal VOC~\cite{pascal-voc-2012}. 

\cite{zhao2019data} have a distinct approach to tackle one-shot segmentation in brain MRIs, where they construct a synthetic dataset from a single labeled image and a large unlabeled dataset using learned transformations via a CNN. This dataset is used in a supervised training of segmentation network.

Although being a few-shot sparse segmentation method, we no present the Guided Nets~\cite{rakelly2018conditional} as a baseline. Even to the best of our efforts, the model did not converge with the episodic training used a single binary dataset(most of the medical datasets used). Thus, it did not seen fair to compare the Guided Nets with our approach.
% In this work we did not present the Guided Nets~\cite{rakelly2018conditional} as a baseline, although being a few-shot sparse segmentation method. There were two main problems with the method. The first, being that using pretrained DNNs from ImageNet datasets were not useful for the medical imaging used. The second, was that even to the best of our efforts, the model did not converge with the episodic training used a single binary dataset(most of the medical datasets used). Since, it did not seen fair to compare the Guided Nets with our approach.
% \todo{Justify the absence of Guided Nets as a baseline: inability to use pretrained DNNs from ImageNet and problems with episodic training on binary labels from the Meta-Dataset (did not converge to the best of our efforts).}

% FIRST VERSION
% Sparse labeling segmentation can be challenging scenario.~\citet{vernaza2017learning} tackle the sparse label scenario in an interesting manner. They propose a labeling propagation scheme using random-walk. Two networks are used, one is used in the labeling propagation and the other is an ordinary segmentation network. In training, in parallel the image is segmented by one of the networks and has the sparse labels propagated to all pixels. The train objective is that these two branches agree on the final prediction.~\citet{cciccek20163d} uses a simple approach to the sparse label scenario. The authors use an UNet architecture in 3d images of \textit{Xenopus} embryos. In this work, to train the network they reweight the importance of the voxels. Voxels of the foreground have an increased impact, while background voxels decrease. Voxels without a label are unconsidered in computing the training loss.

% Our work is uses the approach of \cite{cciccek20163d}, to deal with sparse labels. Our methods are built upon MAML \cite{finn2017model} and ProtoNets \cite{snell2017prototypical}, thus is related to CITE. The frameworks of MAML and ProtoNets will be further detailed in the section CITE, since they are essential to our methods.

% \subsection{Few-Shot Segmentation from Sparse Labels}
% \label{sec:few_shot_sparse_seg}

% % "This is a natural extension of [24] to segmentation, but we find it is difficult to optimize for structured output, perhaps due to multi-modality or fine-tuning from pre-training. [...] In comparing feature fusion, parameter regression, and prototypes we find feature fusion is more accurate and simpler to tune. This is the inference strategy used for all of our results." \cite{rakelly2018conditional}.

% All methods referenced in Section~\ref{sec:few_shot_seg} address the problem of few-shot semantic segmentation regarding the number of labeled images used in the support set, while the methods presented in Section~\ref{sec:sparse_seg}. However, none of these methods address the scenario of few-shot learning from sparse annotations, relying on laborious dense labeling masks. Dense masks may be unfeasible or undesirable for applications that depend on annotations from specialists (e.g. biomedical imaging or remote sensing).

% \cite{rakelly2018conditional} proposed the first algorithm for few-shot sparse segmentation.

% The authors of \cite{rakelly2018conditional} use the same network to extract features of the support set and the query image, but the support features are used as weights.
